Adaptation of the Independent Metropolis-Hastings Sampler with Normalizing Flow Proposals

Markov Chain Monte Carlo (MCMC) methods are a powerful tool for computation with complex probability distributions. However the performance of such methods is critically dependant on properly tuned parameters, most of which are difficult if not impossible to know a priori for a given target distribution. Adaptive MCMC methods aim to address this by allowing the parameters to be updated during sampling based on previous samples from the chain at the expense of requiring a new theoretical analysis to ensure convergence. In this work we extend the convergence theory of adaptive MCMC methods to a new class of methods built on a powerful class of parametric density estimators known as normalizing flows. In particular, we consider an independent Metropolis-Hastings sampler where the proposal distribution is represented by a normalizing flow whose parameters are updated using stochastic gradient descent. We explore the practical performance of this procedure on both synthetic settings and in the analysis of a physical field system and compare it against both adaptive and non-adaptive MCMC methods.

==> Adaptation of the Independent Metropolis-Hastings Sampler with Normalizing Flow Proposals/algorithms/independent-adaptive.tex <==
\begin{algorithm}[t!]
  \caption{Algorithm for sampling from a target distribution by adapting a normalizing flow proposal distribution in the independent Metropolis-Hastings algorithm using the pseudo-likelihood objective.}
  \label{alg:pseudo-likelihood-adaptive}
  \begin{algorithmic}
    \STATE {\bf Input:} A sequence of step-sizes $(\epsilon_0,\epsilon_1,\ldots)$; a sequence of adaptation probabilities $(\alpha_0, \alpha, \ldots)$ an initial state $x_0$ and initial parameter $\theta_0$; a target distribution with density $\pi : \mathcal{X}\to\R$.
    \FOR{$n = 0,1,2,\ldots$}
    \STATE Sample a proposal state from the current proposal distribution $\tilde{x}_{n+1} \sim \tilde{\Pi}_{\theta_{n-1}}$.
    \STATE Generate $u\sim \mathrm{Uniform}(0, 1)$ and compute the Metropolis-Hastings accept-reject decision.
    \begin{align}
        a \gets u < \min\set{1, \frac{\pi(\tilde{x}_{n+1}) \tilde{\pi}_{\theta_{n}}(x_{n})}{\pi(x_{n})\tilde{\pi}_{\theta_{n}}(\tilde{x}_{n+1})}}
    \end{align}
    \IF{$a$}
    \STATE Accept the proposal $x_{n+1}\gets \tilde{x}_{n+1}$.
    \ELSE 
    \STATE Remain at current state $x_{n+1} \gets x_{n}$.
    \ENDIF
    \STATE Generate $u' \sim \mathrm{Uniform}(0, 1)$.
    \IF{$u' < \alpha_n$}
    \STATE Update the parameters
    \begin{align}
        \theta_{n+1} \gets \theta_n + \epsilon_n \nabla \log \tilde{\pi}_{\theta_n}(x_k)
    \end{align}
    where $k\sim\mathrm{Uniform}(\set{0,1\ldots, n+1})$.
    \ELSE
    \STATE Otherwise, keep the current parameters $\theta_{n+1}\gets \theta_n$.
    \ENDIF
    \ENDFOR
  \end{algorithmic}
\end{algorithm}
% \begin{algorithm}[t!]
%   \caption{Algorithm for the independent adaptation of a parameterizable density $\tilde{\pi}_{\theta}$ for use in the independent Metropolis-Hastings algorithm. Since adaptations are independent by construction, this theory is equipped by an ergodicity theory; see \citet{adaptive-independent-metropolis}. Moreover, the stationary distribution of the chain is the target density.}
%   \label{alg:independent-adaptive}
%   \begin{algorithmic}
%     \STATE {\bf Input:} An adaptation function $L : \mathcal{Y}\times\R \times (\cdot)\to\mathcal{Y}$ to adapt the parameters of the normalizing flow; a sequence of step-sizes $(\epsilon_0,\epsilon_1,\ldots)$; an initial state $x_0$ and initial parameter $\theta_0$; a target distribution with density $\pi : \mathcal{X}\to\R$.
%     \FOR{$n = 0,1,2,\ldots$}
%     \IF{Global updates}
%     \STATE Sample a proposal state from the current proposal distribution $\tilde{x}_{n+1} \sim \tilde{\Pi}_{\theta_{n-1}}$.
%     \STATE Generate $u\sim \mathrm{Uniform}(0, 1)$ and compute the Metropolis-Hastings accept-reject decision.
%     \begin{align}
%         a \gets u < \min\set{1, \frac{\pi(\tilde{x}_{n+1}) \tilde{\pi}_{\theta_{n}}(x_{n})}{\pi(x_{n})\tilde{\pi}_{\theta_{n}}(\tilde{x}_{n+1})}}
%     \end{align}
%     \IF{$a$}
%     \STATE Accept the proposal $x_{n+1}\gets \tilde{x}_{n+1}$.
%     \STATE Update the history with the current state $\mathcal{H}_{n+1} \gets \mathcal{H}_n \cup \set{x_n}$.
%     \ELSE 
%     \STATE Remain at current state $x_{n+1} \gets x_{n}$.
%     \STATE Update the history with the proposal state $\mathcal{H}_{n+1} \gets \mathcal{H}_n \cup \set{\tilde{x}_{n+1}}$.
%     \ENDIF
%     \STATE Update parameters 
%     \begin{align}
%         \theta_{n+1} \gets \theta_n + L(\theta_n, \epsilon_n, \mathcal{H}_n, \epsilon_n).
%     \end{align}
%     \ELSIF{Local updates (MALA, HMC, etc.)}
%     \STATE $x_{n+1} \gets \cdots$.
%     \STATE Information based on local updates cannot be used to update parameters.
%     \begin{align}
%         \mathcal{H}_{n+1} &\gets \mathcal{H}_n \\
%         \theta_{n+1} &\gets \theta_n.
%     \end{align}
%     \ENDIF
%     \ENDFOR
%   \end{algorithmic}
% \end{algorithm}


==> Adaptation of the Independent Metropolis-Hastings Sampler with Normalizing Flow Proposals/appendices/adaptation-kl-divergence-flow.tex <==
\clearpage
\section{Adaptation via the Flow of the KL Divergence}

Consider an adaptive sequence of parameters $(\theta_0,\theta_1,\ldots)$ which parameterize proposal densities $(\tilde{\pi}_{\theta_0},\tilde{\pi}_{\theta_1},\ldots)$. Given a target distribution $\Pi$ with density $\pi$, the efficacy of the adaptive independent Metropolis-Hastings sampler is dictated by the ratio of the target density to the proposal density,
\begin{align}
    \label{eq:least-upper-bound-ratio} U(\theta) \defeq \sup_{x\in \mathrm{Supp}(\pi)} \frac{\pi(x)}{\tilde{\pi}_{\theta}(x)}.
\end{align}
The smaller this upper bound, the better the mixing properties of the independent Metropolis-Hastings algorithm with proposal distribution $\tilde{\Pi}_{\theta_n}$. A central question is whether or not the sequence $(\theta_0,\theta_1,\ldots)$ actually produces improvements in these upper bounds; i.e. is $U(\theta_{n+1}) \leq U(\theta_n)$?

It is important that the bound in \cref{eq:least-upper-bound-ratio} is actually the {\it least} upper bound. This is because an arbitrary upper bound may decrease while the least upper bound decreases.

In estimating the parameters of normalizing flows, it is typical that parameters follow, at least approximately, the gradient flow of a prescribed loss function, such as a KL divergence. Since gradient flows are initial value problems with deterministic solutions, by examining the case wherein adaptations are obtained exactly by gradient flow allows us to bypass the added difficulty of contending with stochastic adaptations. 
\begin{proposition}\label{prop:flow-descent-direction}
Let $\mathcal{X}$ be a state space and let $\theta\in\R^m$ parameterize a probability measure $\tilde{\Pi}_\theta$ on $\mathfrak{B}(\mathcal{X})$ with density $\tilde{\pi}_\theta$. Given a target density $\pi$, consider the function $U : \R^m\to\R$ defined by \cref{eq:least-upper-bound-ratio} and assume further that $U$ is smooth with respect to its argument. Let $L : \R^m\to\R$ be a loss function and consider the gradient flow $\theta_t = - \nabla L(\theta_t)$ given an initial condition $\theta_0$. A sufficient condition that $U(\theta_{t+s}) \leq U(\theta_t)$ is that
\begin{align}
    \nabla U(\theta_{t'}) \cdot \nabla L(\theta_{t'}) \geq 0,
\end{align}
where $t'\in (t, t+s)$; i.e. $\nabla L(\theta_{t'})$ is an ascent direction of $U$ at $\theta_{t'}$.
\end{proposition}
\begin{proof}
By applying the chain rule,
\begin{align}
    \frac{\mathrm{d}}{\mathrm{d}t} U(\theta_t) &= \nabla U(\theta_t) \cdot \dot{\theta}_t \\
    &= \nabla U(\theta_t) \cdot -\nabla L(\theta_t).
\end{align}
By the fundamental theorem of calculus,
\begin{align}
    U(\theta_{t+s}) - U(\theta_t) &= \int_t^{t+s} \paren{\frac{\mathrm{d}}{\mathrm{d}t'} U(\theta_{t'})}\bigg|_{t' = t''} ~\mathrm{d}t'' \\
    &= -\int_t^{t+s} \nabla U(\theta_{t''}) \cdot \nabla L(\theta_{t''}) ~\mathrm{d}t'' \\
    &\leq 0
\end{align}
Therefore, $U(\theta_{t+s}) \leq U(\theta_t)$.
\end{proof}
While verifying the conditions of \cref{prop:flow-descent-direction} in general appears a daunting task, we can do some analysis in simple cases.
\begin{example}
Consider the problem of sampling $\mathrm{Normal}(0, 1)$ by adapting a proposal of the form $\mathrm{Normal}(\mu, \sigma^2)$. Assume further that $\sigma^2 > 1$. We can deduce a an upper bound on the ratio of the target density to the proposal density as follows:
\begin{align}
    \max_{x\in \R} \frac{\exp(-x^2/2) / \sqrt{2\pi}}{\exp(-(x-\mu)^2 / 2\sigma^2) / \sqrt{2\pi\sigma^2}} &= \sigma \max_{x\in \R} \exp\paren{-\frac{x^2}{2} + \frac{(x-\mu)^2}{2\sigma^2}} \\
    \label{eq:gaussian-upper-bound} &\leq \sigma \exp\paren{\frac{\mu^2}{2(\sigma^2 - 1)}},
\end{align}
which can be deduced by maximizing $-\frac{x^2}{2} + \frac{(x-\mu)^2}{2\sigma^2}$ using calculus. The reverse KL divergence between the proposal distribution and the target distribution is seen to be,
\begin{align}
    \mathbb{KL}(\mathrm{Normal}(\mu, \sigma^2)\Vert \mathrm{Normal}(0, 1)) = -\log\sigma + \frac{\sigma^2 + \mu^2}{2} - \frac{1}{2}.
\end{align}
Consider the gradient flow of the reverse KL divergence:
\begin{align}
    \dot{\mu}_t  &= -\frac{\partial}{\partial\mu} \mathbb{KL}(\mathrm{Normal}(\mu, \sigma^2)\Vert \mathrm{Normal}(0, 1)) \\
    &= -\mu \\
    \dot{\sigma}_t &= -\frac{\partial}{\partial \sigma}\mathbb{KL}(\mathrm{Normal}(\mu, \sigma^2)\Vert \mathrm{Normal}(0, 1)) \\
    &= \frac{1}{\sigma_t} - \sigma_t.
\end{align}
When we specify initial conditions $\mu_0\in\R$ and $\sigma_0 > 1$, this produces an initial value problem.
To verify that adapting by following the gradient flow of KL divergence produces a provable improvement to the upper bound deduced in \cref{eq:gaussian-upper-bound}, it suffices to check that the time derivative of the upper bound in decreasing under the postulated gradient flow dynamics. That is,
\begin{align}
\begin{split}
    \frac{\mathrm{d}}{\mathrm{d}t} \sigma_t \exp\paren{\frac{\mu_t^2}{2(\sigma^2_t - 1)}} &= \frac{\mu_t\sigma_t \exp(\mu_t^2 / (2(\sigma^2_t - 1)))}{\sigma_t^2 - 1} \cdot -\mu_t \\
    &\qquad +~ \frac{\exp(\mu_t^2 / (2(\sigma^2_t - 1)))(-(\mu_t^2+2)\sigma_t^2 + \sigma_t^4 + 1)}{(\sigma_t^2 - 1)^2} \cdot \paren{\frac{1}{\sigma_t} - \sigma_t}
\end{split} \\
&= - \frac{(\sigma_t - 1)(\sigma_t + 1)\exp(\mu_t^2 / (2(\sigma^2_t - 1)))}{\sigma_t}.
\end{align}
It follows that this is a negative quantity if we can establish that $\sigma_t > 1$. From the initial condition $\sigma_0>1$, it follows that the positive solution of the differential equation $\dot{\sigma}_t = \frac{1}{\sigma_t} - \sigma_t$ is $\sigma_t = \sqrt{e^{-2t}(\sigma_0^2-1) + 1}$, so we see, indeed, that $\sigma_t > 1$. Therefore, the upper bound is a decreasing function of $t$ given the prescribed gradient flow dynamics. The differential equation $\dot{\mu}_t = -\mu_t$ also has an explicit solution given the initial condition $\mu_0$, which is $\mu_t = \mu_0 e^{-t}$. These explicit solutions to the gradient flow of the KL divergence allow us to express the evolution of the upper bound concretely as,
\begin{align}
    \sqrt{e^{-2t}(\sigma_0^2-1) + 1}\exp\paren{\frac{\mu_0^2 e^{-2t}}{2e^{-2t}(\sigma_0^2-1)}} = \sqrt{e^{-2t}(\sigma_0^2-1) + 1}\exp\paren{\frac{\mu_0^2 }{2(\sigma_0^2-1)}}
\end{align}
This is an intriguing formula since it suggests that although the sequence $M_{t}$ is decreasing, it decreases only to a non-unit limit $\exp(\mu_0^2 / (2(\sigma_0^2 - 1)))$; indeed, unless $\mu_0 =0$, the limit of this upper bound does not approach one. For the purposes of MCMC, this may be acceptable, since uniform ergodicity can be obtained so long as the bound is finite; however, were the upper bound to equal one, this would be optimal.
Connecting this back to the question of adaptation, choosing an increasing sequence of times $t_0< t_1<t_2<\ldots$ and consider using $\mathrm{Normal}(\mu_{t_n}, \sigma^2_{t_n})$ as the proposal distribution at step $n$. The Doeblin coefficient at step $n$ is therefore,
\begin{align}
    L_n = \frac{1}{\sqrt{e^{-2t}(\sigma_0^2-1) + 1}\exp\paren{\frac{\mu_0^2}{2(\sigma_0^2-1)}}}.
\end{align}
Finally, let us remark that the undesirable property that the upper bounds do not converge to unity can be easily corrected. The principle issue is that the factors of $e^{-2t}$ cancel in the exponent. However, consider that instead of the using $(\mu_t,\sigma_t)$ to inform adaptations one instead uses $(\mu_{2t}, \sigma_t)$ so that the mean value is further along in the solution to its initial value problem than the scale. Plugging this into the formula for the upper bound yields,
\begin{align}
    \sqrt{e^{-2t}(\sigma_0^2-1) + 1}\exp\paren{\frac{\mu_0^2 e^{-4t}}{2e^{-2t}(\sigma_0^2-1)}} =  \sqrt{e^{-2t}(\sigma_0^2-1) + 1}\exp\paren{\frac{\mu_0^2 e^{-2t}}{2(\sigma_0^2-1)}},
\end{align}
which converges to unity as $t\to\infty$ as desired.

Instead of the reverse KL divergence we may consider the forward KL divergence between the target distribution and the proposal.
\begin{align}
    \mathbb{KL}(\mathrm{Normal}(0, 1)\Vert \mathrm{Normal}(\mu, \sigma^2)) = \log\sigma + \frac{1 + \mu^2}{2\sigma^2} - \frac{1}{2}.
\end{align}
The forward KL divergence produces the following equations of motion.
\begin{align}
    \dot{\mu}_t &= -\frac{\mu_t}{\sigma_t^2} \\
    \dot{\sigma}_t &= \frac{\mu_t^2 + 1}{\sigma_t^3} - \frac{1}{\sigma_t}
\end{align}
Applying the chain rule to \cref{eq:gaussian-upper-bound} with these equations of motion yields the following time derivative of the upper bound,
\begin{align}
    \frac{\mathrm{d}}{\mathrm{d}t} \sigma_t \exp\paren{\frac{\mu_t^2}{2(\sigma_t^2 - 1)}} = \exp\paren{\frac{\mu_t^2}{2(\sigma_t^2 - 1)}} \frac{-\mu_t^4 \sigma^2 + \mu_t^2\sigma_t^4 - 2\mu_t^2\sigma_t^2 + \mu_t^2 - \sigma_t^6 + 3\sigma_t^4 - 3\sigma_t^2 + 1}{\sigma_t^3(\sigma_t^2 - 1)^2}.
\end{align}
This derivative is less than or equal to zero iff
\begin{align}
    &-\mu_t^4 \sigma^2 + \mu_t^2\sigma_t^4 - 2\mu_t^2\sigma_t^2 + \mu_t^2 - \sigma_t^6 + 3\sigma_t^4 - 3\sigma_t^2 + 1 \leq 0 \\
    \iff & \mu_t^2(\sigma_t^2 - 1)^2 \leq \mu_t^4 \sigma_t^2 + (\sigma_t^2 - 1)^3,
\end{align}
which is true for $\sigma_t^2 > 1$. 

\end{example}

==> Adaptation of the Independent Metropolis-Hastings Sampler with Normalizing Flow Proposals/appendices/exp-field.tex <==
\clearpage
\section{Experimental details on field experiment}
\label{app:exp-field}

We provide additional details on the experiment presented in \cref{sec:phi4}. 

\paragraph{Field distribution.} The $\phi^4$ field model is a popular model used to study phase transition in statistical mechanics (see for example \citep{berglund_eyring_2017}). Here we focus on its $1d$ version, where is field is defined on the segment $[0,1]$, and impose Dirichlet boundary conditions $\phi(0)=\phi(1) = 0$. 
The energy function is an intergral over the segment of two terms:
\begin{align}
    \label{eq:phi4-app}
    U(\phi) = \int_0^1   \left[ \frac{a}{2} (\partial_s \phi )^2 + \frac{1}{4a}\left(1-\phi^2(s)\right)^2  \right] \mathrm{d}s.
\end{align}
The \emph{coupling term} $\frac{a}{2} (\partial_s \phi )^2$ encourages the smoothness of the field, while the local potential term $\frac{1}{4a}\left(1-\phi^2(s)\right)^2$ favors fields taking values close to $1$ or $-1$ over the segment. 
For large values of the parameter $a$, fields with significant statistical weights will take values close to $0$ over the entire segment $[0,1]$. As $a$ decreases, the system undergoes a \emph{phase transition} and two distinct modes forms concentrating around either $+1$ or $-1$. 

Note that here the energy function \eqref{eq:phi4-app} is symmetric under the symmetry $\phi \to - \phi$. We exploit this symmetry to provide high-quality reference samples in the experiments described next. Note however that as a biasing term is added to the energy, the statistical weights of either of the mode becomes unknown. 

The numerical experiments described next shows that the adaptive sampler with normalizing flow proposals can recover the relative statistics thanks to efficient mixing, at least at the level of discretization described. Conversely, the energy barrier between the two modes prevents a Langevin sampler from mixing in a reasonable time.

\paragraph{Numerics.} We sample the field at 100 equally spaced locations between $0$ and $1$. The RealNVP flow \citep{DBLP:conf/iclr/DinhSB17} we optimize has $5$ pairs of affine coupling layers updating each half of the $100$ field variables. The scaling and translation transformations of each coupling layer is a 2-hidden-layer perceptron with relu activations and $100$ units per layer.

The algorithm minimizing the ``pseudo-likelihood'' objective, defined in Example \cref{ex:normalizing-flow-pseudo-lkl}, follows largely the lines of \cref{alg:pseudo-likelihood-adaptive}. Being more specific, we collect the states of $100$ parallel walkers every $10$ sampling iterations and take a gradient step with the corresponding $1000$-sample batch. The initial learning rate of $10^{-3}$ is halved every $5000$ gradient steps.

We initialize $100$ chains: $20$ at the uniform value of $1$ and $80$ at the uniform value of $-1$.
Thanks to the adaptation of the normalizing flow, leading to good acceptance as reported in the main text, these chains can easily mix between modes and recover the proper statistical weights of $50/50$. 

\input{figures/field-model-samples}




==> Adaptation of the Independent Metropolis-Hastings Sampler with Normalizing Flow Proposals/appendices/kernel-density-adaptation.tex <==
\clearpage
\section{Adaptation of a Kernel Density Proposal Distribution}

A principle difficulty in using normalizing flows as proposal distributions is that it is unclear whether or not a given adaptation of the neural network parameters will provably decrease the upper bound on the ratio of the target density and the normalizing flow density. Analyzing this property theoretically in the case of normalizing flows does not appear to be forthcoming. Nevertheless, we have been able to analyze certain behaviors of proposals based on kernel density estimators. A version of this procedure (to use kernel density estimators as a proposal in independent Metropolis-Hastings) was previously pursued in \citet{doi:10.1080/10618600.2019.1598872}; however, they do not appear to have looked at the question of when the addition of a new component into the mixture is beneficial, which is the topic under consideration in the sequel.

Let $x_1,\ldots,x_n\in\R^m$. We consider the kernel density estimator computed by,
\begin{align}
    \tilde{K}_n(x) &= \frac{1}{n} \sum_{i=1}^n \frac{1}{\mathrm{Vol}(\bar{B}_{\epsilon}(x_i))} \mathbf{1}\set{x \in \bar{B}_{\epsilon}(x_i)}.
\end{align}
where $\bar{B}_\epsilon(x)$ is the closed ball of radius $\epsilon$ centered at $x$. For notational convenience, we observe that $V = \mathrm{Vol}(\bar{B}_{\epsilon}(x)) = \mathrm{Vol}(\bar{B}_{\epsilon}(x'))$ for any $x,x'\in \R^m$ and we write $m_n(x) = \#\set{i\in (1, \ldots, n) : x \in \bar{B}_{\epsilon}(x_i)}$. Therefore, we have the simple expression for the kernel density estimator as $\tilde{K}_n(x) = m_n(x) / nV$.

Suppose that $\Pi$ is a probability measure on $\R^m$ with compactly supported density $\pi :\R^m\to\R_+$. Define,
\begin{align}
    M_n &=  n V \sup_{x\in\mathrm{Supp}(\pi)} \frac{\pi(x)}{m_n(x)}
\end{align}
Hence $\pi(x) / \tilde{K}_n(x) \leq M_n$.
Given a new observation $x_{n+1}\in\R^m$, we would like to understand conditions under which one can show $M_{n+1} \leq M_n$. This means that the inclusion of a new observation in the kernel density estimate reduces the upper bound on the ratio of the target density and the proposal density. To discuss this, we begin with two definitions.
\begin{definition}
The inner bound is defined by,
\begin{align}
    M_n' = \sup_{x\in \bar{B}_\epsilon(x_{n+1})\cap\mathrm{Supp}(\pi)} \frac{\pi(x)}{m_n(x)}.
\end{align}
\end{definition}
\begin{definition}
The outer bound is defined by,
\begin{align}
    M_n'' = \sup_{x\in \mathrm{Supp}(\pi) \setminus \bar{B}_\epsilon(x_{n+1})} \frac{\pi(x)}{m_n(x)}.
\end{align}
\end{definition}

\begin{lemma}\label{lem:max-supremum}
Let $A$ and $B$ be sets. Then $\max\set{\sup A, \sup B} = \sup A\cup B$.
\end{lemma}
\begin{proof}
Since $A\subset A\cup B$, it is immediate that $\sup A \leq \sup A\cup B$. Identical reasoning shows that $\sup B\leq \sup A\cup B$. Therefore, $\max\set{\sup A, \sup B} \leq \sup A\cup B$. Now suppose without loss of generality that $\sup B\geq \sup A$. Then for all $a\in A$ we have $a \leq \sup B$; moreover, for all $b\in B$, $b \leq \sup B$. Therefore, for all $x\in A\cup B$, $x\leq \sup B$. Thus, $\sup A\cup B \leq \sup B$, since $\sup A \cup B$ is by definition the least upper bound. Applying identical reasoning to the case $\sup A\geq \sup B$ reveals $\sup A\cup B\leq \max\set{\sup A, \sup B}$. Thus, we must have $\sup A\cup B = \max\set{\sup A, \sup B}$.
\end{proof}
\begin{corollary}
Since $\mathrm{Supp}(\pi)\setminus \bar{B}_\epsilon(x_{n+1})= \mathrm{Supp}(\pi) \cap \bar{B}_\epsilon(x_{n+1})^\mathrm{c}$, it follows from the distributive law of set relationships that,
\begin{align}
    \set{\mathrm{Supp}(\pi) \cap \bar{B}_\epsilon(x_{n+1})} \cup \set{\mathrm{Supp}(\pi)\setminus \bar{B}_\epsilon(x_{n+1})} = \mathrm{Supp}(\pi).
\end{align}
Applying \cref{lem:max-supremum} shows that $n V \max\set{M_n', M_n''} = M_n$.
\end{corollary}

\begin{lemma}
The kernel density estimator $\tilde{K}_{n+1}(x)$ can be written as,
\begin{align}
    \tilde{K}_{n+1}(x) = \begin{cases}
        \frac{m_n(x)}{(n+1)V} & ~\mathrm{if}~ x\not\in \bar{B}_\epsilon(x_{n+1}) \\
        \frac{m_n(x) + 1}{(n+1)V} & ~\mathrm{otherwise}.
    \end{cases}
\end{align}
\end{lemma}
\begin{proof}
This follows immediately from the equation,
\begin{align}
    \tilde{K}_{n+1}(x) &= \frac{1}{(n+1)V} \sum_{i=1}^{n+1} \mathbf{1}\set{x\in \bar{B}_\epsilon(x_{i})} \\
    &= \frac{1}{(n+1)V} \paren{m_n(x) + \mathbf{1}\set{x\in\bar{B}_\epsilon(x_{n+1})}}.
\end{align}
\end{proof}

\begin{lemma}\label{lem:outer-bound}
We have,
\begin{align}
    \sup_{x\in \mathrm{Supp}(\pi) \setminus \bar{B}_\epsilon(x_{n+1})}\frac{\pi(x)}{\tilde{K}_{n+1}(x)} = (n+1) V M_n''.
\end{align}
\end{lemma}
\begin{proof}
For $x\in \mathrm{Supp}(\pi) \setminus \bar{B}_\epsilon(x_{n+1})$,
\begin{align}
    \frac{\pi(x)}{\tilde{K}_{n+1}(x)} = (n+1) V \frac{\pi(x)}{m_n(x)}.
\end{align}
Therefore,
\begin{align}
    \sup_{x\in \mathrm{Supp}(\pi) \setminus \bar{B}_\epsilon(x_{n+1})} \frac{\pi(x)}{\tilde{K}_{n+1}(x)} &= (n+1) V \sup_{x\in \mathrm{Supp}(\pi) \setminus \bar{B}_\epsilon(x_{n+1})} \frac{\pi(x)}{m_n(x)} \\
    &= (n+1)V M_n''.
\end{align}
\end{proof}
\begin{lemma}\label{lem:inner-bound}
We have,
\begin{align}
    \sup_{x \in \mathrm{Supp}(\pi)\cap \bar{B}_\epsilon(x_{n+1})} \frac{\pi(x)}{\tilde{K}_{n+1}(x)} \leq nV Q_n M_n',
\end{align}
where
\begin{align}
    Q_n = \sup_{x\in \mathrm{Supp}(\pi)\cap \bar{B}_\epsilon(x_{n+1})} \frac{m_n(x) (n+1)}{(m_n(x) + 1)n} \leq 1.
\end{align}
\end{lemma}
\begin{proof}
Within $ \mathrm{Supp}(\pi)\cap \bar{B}_\epsilon(x_{n+1})$ we have the bound,
\begin{align}
    & nV \frac{\pi(x)}{m_n(x)} \leq nV M_n' \\
    \implies& \frac{\pi(x)}{m_n(x) / nV} \cdot \frac{m_n(x) / n}{(m_n(x) + 1) / (n+1)} \leq \frac{m_n(x) / n}{(m_n(x) + 1) / (n+1)} nV M_n' \\
    \implies& \frac{\pi(x)}{\tilde{K}_{n+1}(x)} \leq nV \frac{m_n(x) / n}{(m_n(x) + 1) / (n+1)}  M_n'
\end{align}
Taking the supremum on both sides yields,
\begin{align}
    \sup_{x \in \mathrm{Supp}(\pi)\cap \bar{B}_\epsilon(x_{n+1})} \frac{\pi(x)}{\tilde{K}_{n+1}(x)} \leq nV Q_n M_n'.
\end{align}
Since $m_n(x)\leq n$, it follows that $Q_n\leq 1$.
\end{proof}

\begin{proposition}\label{prop:larger-exterior-no-improvement}
If $M_n'' > M_n'$, then $M_{n+1} > M_n$. In this case, the inclusion of the new observation degrades the quality of the proposal distribution.
\end{proposition}
\begin{proof}
Since $M_n'' > M_n'$, it follows that
\begin{align}
    \sup_{x\in \mathrm{Supp}(\pi)\cap \bar{B}_\epsilon(x_{n+1})} \frac{\pi(x)}{\tilde{K}_{n+1}(x)} &\leq nV Q_n M_n' \\
    &\leq nV M_n' \\
    &< nV M_n'' \\
    &\leq (n+1)V M_n'' \\
    &= \sup_{x\in \mathrm{Supp}(\pi)\setminus \bar{B}_\epsilon(x_{n+1})} \frac{\pi(x)}{\tilde{K}_{n+1}(x)}.
\end{align}
Hence $M_{n+1} = (n+1)VM_n'' > nVM_n'' = M_n$.
\end{proof}
\begin{proposition}\label{prop:necessary-and-sufficient-kernel-proposal}
It is necessary and sufficient that $(1 + 1/n) M''_n \leq M_n'$ in order for $M_{n+1}\leq M_n$.
\end{proposition}
\begin{proof}
To establish sufficiency, we have:
\begin{align}
    M_{n+1} &\leq \max\set{(n+1) VM_n'', nVQ_n M_n'} \\
    &\leq \max\set{nVM_n', nVQ_n M_n'} \\
    &= nVM_n' \\
    &= M_n
\end{align}
To show that this is actually necessary, consider $M_n'' \leq M_n' < (1 + 1/n) M_n''$. Then, from \cref{lem:outer-bound} we know,
\begin{align}
    \sup_{x\in \mathrm{Supp}(\pi) \setminus \bar{B}_\epsilon(x_{n+1})}\frac{\pi(x)}{\tilde{K}_{n+1}(x)} = (n+1) V M_n''.
\end{align}
But from \cref{lem:inner-bound} we have,
\begin{align}
    \sup_{x \in \mathrm{Supp}(\pi)\cap \bar{B}_\epsilon(x_{n+1})} \frac{\pi(x)}{\tilde{K}_{n+1}(x)} &\leq nV Q_n M_n' \\
    &< (n+1)VQ_n M_n'' \\
    &\leq (n+1)VM_n''
\end{align}
Now $M_n = nVM_n' < (n+1)VM_n'' = M_{n+1}$.
\end{proof}

\Cref{prop:larger-exterior-no-improvement} informs us that if the worst case bound is outside of $\bar{B}_\epsilon(x_{n+1})$, then the adaptation has actually made the bound worse. This is because the density outside of $\bar{B}_\epsilon(x_{n+1})$ behaves in a predictable manner: it is decreased by a factor of $n / (n+1)$. Therefore, if the worst case bound on the ratio occurs outside of $\bar{B}_\epsilon(x_{n+1})$, the ratio can only get worse. At the same time, \cref{prop:necessary-and-sufficient-kernel-proposal} informs us that the worst-case bound on the ratio inside $\bar{B}_\epsilon(x_{n+1})$ must be greater than the worst-case bound outside of $\bar{B}_\epsilon(x_{n+1})$ by at least a factor of $(1 + 1/n)$ in order for the inclusion of the additional observation $x_{n+1}$ to improve the worst-case bound of the ratio of the target density to the kernel density estimator.


==> Adaptation of the Independent Metropolis-Hastings Sampler with Normalizing Flow Proposals/appendices/mixture-kernel-diminishing-adaptation-containment.tex <==
\clearpage
\section{Diminishing Adaptation and Containment for Mixture Kernels}
\label{app:mixture-kernels}
\begin{proposition}\label{prop:containment-from-doeblin}
Let $\Pi$ be a probability measure with density $\pi$ with respect to measure $\mu$. Let $\theta\in\mathcal{Y}$ and suppose that $\theta$ parameterizes a transition kernel $K_{\theta}$. Let $(\Theta_0,\Theta_1,\ldots)$ be a sequence of $\mathcal{Y}$-valued random variables.
Suppose that with probability $1-\delta$ there exists $M\equiv M(\delta)\in\mathbb{N}$ such that $K_{\Theta_n}(x, \mathrm{d}x') \geq \frac{\pi(x')}{M} \mu(\mathrm{d}x')$ for every $n=1,2,\ldots$. Then $(K_{\Theta_0},K_{\Theta_1},\ldots)$ exhibits containment.
\end{proposition}
\begin{proof}
By assumption, with probability $1-\delta$, there exists $M\equiv M(\delta)\in\mathbb{N}$ such that $K_{\Theta_n}(x, \mathrm{d}x') \geq \frac{\pi(x')}{M} \mu(\mathrm{d}x')$ for every $n=1,2,\ldots$ and any $x\in\mathcal{X}$. Therefore, with probability $1-\delta$, there exists $M\equiv M(\delta)\in\mathbb{N}$ such that,
\begin{align}
    \Vert K^m_{\Theta_n}(x, \cdot) -\Pi(\cdot)\Vert_{\mathrm{TV}} \leq \paren{1 - \frac{1}{M}}^m
\end{align}
for any $m\in\mathbb{N}$, every $n=1,2,\ldots$, and $x\in \mathcal{X}$. Let $\epsilon > 0$ be arbitrary. Then, with probability $1-\delta$, there exists $N=N(\epsilon,\delta)\in\mathbb{N}$ such that
\begin{align}
    \Vert K^N_{\Theta_n}(x, \cdot) - \Pi(\cdot)\Vert_{\mathrm{TV}} \leq \epsilon.
\end{align}
for every $n=1,2,\ldots$ and any $x\in \mathcal{X}$. Namely, the choice
\begin{align}
    N(\epsilon,\delta) = \ceil[\Bigg]{\frac{\log \epsilon}{\log\paren{1 - \frac{1}{M(\delta)}}}}
\end{align}
suffices. Thus as a special case, with probability $1-\delta$, there exists $N=N(\epsilon,\delta)\in\mathbb{N}$ such that
\begin{align}
    \Vert K^N_{\Theta_n}(X_n, \cdot) - \Pi(\cdot)\Vert_{\mathrm{TV}} \leq \epsilon.
\end{align}
for every $n=1,2,\ldots$. Define the function,
\begin{align}
    W_\epsilon(x, \theta) = \inf \set{n\in \mathbb{N} : \Vert K_\theta^n(x, \cdot) - \Pi(\cdot)\Vert_{\mathrm{TV}} \leq \epsilon}.
\end{align}
Hence, with probability $1-\delta$, there exists $N=N(\epsilon,\delta)\in\mathbb{N}$ such that
\begin{align}
    W_\epsilon(X_n, \Theta_n) \leq N
\end{align}
for every $n=1,2,\ldots$. This is the containment condition.
\end{proof}

\begin{proposition}
Let $\Pi$ be probability measure with density $\pi$ with respect to measure $\mu$. Let $\theta\in\mathcal{Y}$ and suppose that $\theta$ parameterizes a probability measure $\tilde{\Pi}_\theta$ with density $\tilde{\pi}_\theta$. Let $K_{\theta}$ be the transition kernel of the independent Metropolis-Hastings sampler of $\Pi$ given $\tilde{\Pi}_{\theta}$:
\begin{align}
    K_{\theta}(x,\mathrm{d}x') = \min\set{1, \frac{\pi(x') \tilde{\pi}_{\theta}(x)}{\pi(x) \tilde{\pi}_{\theta}(x')}} \tilde{\pi}_{\theta}(x') ~\mu(\mathrm{d}x') + \paren{1 - \int_{\mathcal{X}} \min\set{1, \frac{\pi(w) \tilde{\pi}_{\theta}(x)}{\pi(x) \tilde{\pi}_{\theta}(w)}} \tilde{\pi}_{\theta}(w) ~\mu(\mathrm{d}w)} \delta_{x}(\mathrm{d}x').
\end{align}
Let $K'$ be another transition and consider the transition kernel that is formed by the mixture of $K_\theta$ and $K'$: $\hat{K}_\theta(x, A) = \alpha K_\theta(x, A) + (1-\alpha) K'(x, A)$ for $x\in \mathcal{X}$ and $A\in\mathfrak{B}(\mathcal{X})$. Let $(\Theta_0,\Theta_1,\ldots)$ be a sequence of $\mathcal{Y}$-valued random variables. If $(K_{\Theta_0}, K_{\Theta_1}, \ldots)$ exhibits diminishing adaptation then so does $(\hat{K}_{\Theta_0},\hat{K}_{\Theta_1},\ldots)$. Furthermore, suppose that with probability at least $1-\delta$ there exists $M\equiv M(\delta)$ such that $K_{\Theta_n}(x, \mathrm{d}x') \geq \frac{\pi(x')}{M} \mu(\mathrm{d}x')$ for every $n=1,2,\ldots$. Then $(\hat{K}_{\Theta_0},\hat{K}_{\Theta_1},\ldots)$ exhibits containment.
\end{proposition}
\begin{proof}
\begin{align}
    d(\hat{K}_{\Theta_n}, \hat{K}_{\Theta_{n+1}}) &= \sup_{x\in\mathcal{X}} \Vert \hat{K}_{\Theta_n}(x, \cdot) - \hat{K}_{\Theta_{n+1}}(x, \cdot)\Vert_{\mathrm{TV}} \\
    &= \sup_{x\in\mathcal{X}} \Vert \alpha K_{\Theta_n}(x, \cdot) - \alpha K_{\Theta_{n+1}}(x, \cdot)\Vert_{\mathrm{TV}} \\
    &= \alpha \sup_{x\in\mathcal{X}} \Vert K_{\Theta_n}(x, \cdot) - K_{\Theta_{n+1}}(x, \cdot)\Vert_{\mathrm{TV}} \\
    &= \alpha d(K_{\Theta_n}, K_{\Theta_{n+1}}).
\end{align}
Hence, if $d(K_{\Theta_n}, K_{\Theta_{n+1}})$ converges in probability to zero then so does $d(\hat{K}_{\Theta_n}, \hat{K}_{\Theta_{n+1}})$.

To show containment, observe that with probability at least $1-\delta$ there exists $M\equiv M(\delta)$ such that,
\begin{align}
    \hat{K}_\theta(x, \mathrm{d}x') &\geq \alpha K_\theta(x, \mathrm{d}x') \\
    &\geq \alpha \frac{\pi(x')}{M} \mu(\mathrm{d}x').
\end{align}
Containment then follows from \cref{prop:containment-from-doeblin}.
\end{proof}


==> Adaptation of the Independent Metropolis-Hastings Sampler with Normalizing Flow Proposals/appendices/non-independent-stationarity.tex <==
\clearpage
\section{Violations of Stationarity}\label{app:violations-of-stationarity}

\input{figures/violations-of-stationarity}

In general, adaptation of the parameters of the transition kernel will destroy stationarity. However, if the adaptations and the state of the chain enjoy a prescribed independence condition, then stationarity of the target distribution can be conserved.
\begin{proposition}\label{prop:stochastic-sequence-stationarity}
  Suppose that $(\Theta_0,\Theta_1,\ldots)$ is a {\it stochastic} $\mathcal{Y}$-valued sequence. Let $(K_{\Theta_n})_{n\in\mathbb{N}}$ be an associated sequence of Markov transition kernels which produces an $\mathcal{X}$-valued chain as $X_{n+1}\sim K_{\Theta_n}(X_n, \cdot)$. Suppose further that $\Theta_n$ and $X_n$ are independent given the history of the chain to step $n-1$. If $\Pi$ is stationary for each $K_{\Theta_n}$, then $\Pi$ is also the stationary distribution of $(X_n)_{n\in\mathbb{N}}$.
\end{proposition}

We first give an illustration of why maximizing the pseudo-likelihood objective may not always be beneficial. In particular, we look for evidence of violations of stationarity; violations of stationarity mean that if one begins with a sample from the target distribution and transforms it according to several steps of the transition kernel with adaptations, then the final state may not be distributed according to the target distribution. This can be interpreted as an undesirable form of sample degradation wherein applications of an adaptive transition kernel move exact samples further from the target distribution.

As a simple example, we consider sampling $\mathrm{Normal}(1, 1/2)$ using a proposal distribution $\mathrm{Normal}(\mu, \sigma^2)$; the proposal distribution can be interpreted as a simple normalizing flow consisting of a shift and scale applied to a standard normal base distribution. We consider adapting the parameters of the proposal distribution by computing the maximum likelihood estimates of the mean and standard deviation using the accepted samples. Specifically, let $(X_0, X_1,\ldots,X_n)$ denote the states of the chain to step $n$; then the parameters of the proposal distribution at step $n+1$ are $\mu_{n+1} = (n+1)^{-1} \sum_{i=0}^n X_i$ and $\sigma_{n+1} = \sqrt{(n+1)^{-1}\sum_{i=0}^n X_i^2 - \mu_{n+1}^2}$. Results for this adaptation mechanism are shown in \cref{fig:stationarity-violation}; after one-hundred steps of adaptation, there is a clear violation of stationarity, but which has nearly vanished by the ten-thousandth step. We observe that adaptations do tend to reduce the forward KL divergence between the target and the proposal distribution, with the closeness improving as the number of adaptation steps increases.

==> Adaptation of the Independent Metropolis-Hastings Sampler with Normalizing Flow Proposals/appendices/product-transition-kernel-independent.tex <==
\clearpage
\section{Independence and Product Transition Kernels}
\label{app:product-kernels}
Let $\Pi$ be a probability measure of $\R^m$ with density $\pi$. Let $\hat{\Pi}(A_1,\ldots, A_n) = \prod_{i=1}^n \Pi(A_i)$ be the product probability measure on $(\R^m)^n = \prod_{i=1}^n \R^m$ (the product space of $n$ copies of $\R^m$). Let $(x_1,\ldots,x_n)\in (\R^m)^n$ and define the $i^\mathrm{th}$ transition kernel by,
\begin{align}
    K_i((x_1,\ldots, x_n), (\mathrm{d}y_1,\ldots,\mathrm{d}y_n)) &= \left[\alpha_i(x_i, y_i) ~\mathrm{d}y_i + \beta_i(x_i)~\delta_{x_i}(\mathrm{d}y_i)\right] \cdot \prod_{j=1,j\neq i}^n \delta_{x_j}(\mathrm{d}y_j) \\
    \alpha_i(x, y) &= \min\set{1, \frac{\pi(y) \tilde{\pi}_i(x\vert y)}{\pi(x) \tilde{\pi}_i(y\vert x)}} \tilde{\pi}_i(y\vert x) \\
    \beta_i(x) &= \paren{1 - \int_{\R^m} \alpha_i(x, w)~\mathrm{d}w}
\end{align}
Thus we can understand $K_i$ as a transition kernel that applies a Metropolis-Hastings accept-reject decision to the $i^\mathrm{th}$ dimension of the posterior using a proposal density $\tilde{\pi}_i(\cdot\vert x_i)$ on $\R^m$ and leaves all other dimensions unchanged. Because of the product structure of the joint distribution, these Metropolis-Hastings updates preserve the joint distribution even though the accept-reject decision is computed only on the $i^\mathrm{th}$ marginal.

As an example, consider $K_1$ and $K_2$. What is the composition transition kernel generated by first applying $K_1$ and subsequently applying $K_2$? By the Chapman-Kolmogorov formula, it is,
\begin{align}
    &(K_2\circ K_1)((x_1,\ldots, x_n), (A_1,\ldots, A_n)) \\
    &= \int_{\R^m} \cdots\int_{\R^m} K_2((y_1,\ldots, y_n), (A_1,\ldots, A_n)) K_1((x_1,\ldots, x_n), (\mathrm{d}y_1,\ldots,\mathrm{d}y_n)) \\
    \begin{split}
    &=\int_{\R^m} \cdots\int_{\R^m} \paren{\left[\int_{A_2} \alpha_2(y_2, w) ~\mathrm{d}w + \beta_2(y_2)~\delta_{y_2}(A_2)\right] \cdot \prod_{j=1,j\neq 2}^n \delta_{y_j}(A_j)} \\
    &\qquad\times ~ \paren{\left[\alpha_1(x_1, y_1) ~\mathrm{d}y_1 + \beta_1(x_1)~\delta_{x_1}(\mathrm{d}y_1)\right] \cdot \prod_{j=1,j\neq 1}^n \delta_{x_j}(\mathrm{d}y_j)}
    \end{split} \\
    &= \left[\int_{A_1} \alpha_1(x_1, w)~\mathrm{d}w + \beta_1(x_1) \delta_{x_1}(A_1)\right]\cdot\left[\int_{A_2} \alpha_2(x_2, w)~\mathrm{d}w + \beta_2(x_2) \delta_{x_2}(A_2)\right] \cdot \prod_{j=3}^n \delta_{x_j}(A_j).
\end{align}
Notice that the composition kernel assumes a factorized form. Suppose that $(x_1',\ldots, x_n') \sim (K_2\circ K_1)((x_1,\ldots, x_n), \cdot)$. Drawing a sample from this composition kernel can be achieved by setting $x'_j = x_j$ for $j=3,\ldots, n$ and sampling $x'_1$ and $x'_2$ independently from the distributions
\begin{align}
    \mathrm{Pr}\left[x'_i \in A\vert x_i\right] = \int_{A} \alpha_i(x_i, w)~\mathrm{d}w + \beta_i(x_i) \delta_{x_i}(A),
\end{align}
for $i\in\set{1, 2}$. 

The fact that any composition kernel $K_k\circ\cdots\circ K_1$ has this product distribution form can be established via induction. Assume
\begin{align}
    (K_k\circ\cdots \circ K_1)((x_1,\ldots, x_n), (\mathrm{d}y_1,\ldots,\mathrm{d}y_n)) = \prod_{i=1}^k \left[\alpha_i(x_i, y_i)~\mathrm{d}y_i + \beta_i(x_i)~\delta_{x_i}(\mathrm{d}y_i)\right] \prod_{j=k+1}^n \delta_{x_j}(\mathrm{d}y_j)
\end{align}
Then,
\begin{align}
    &(K_{k+1}\circ\cdots\circ K_1)((x_1,\ldots, x_n), (A_1,\ldots, A_n)) \\
    &= \int_{(\R^m)^n} K_{k+1}((y_1,\ldots, y_n), (A_1,\ldots, A_n)) (K_k\circ\cdots \circ K_1)((x_1,\ldots, x_n), (\mathrm{d}y_1,\ldots,\mathrm{d}y_n)) \\
    \begin{split}
    &= \int_{(\R^m)^n} \left[\paren{\int_{A_{k+1}} \alpha_{k+1}(y_{k+1}, w)~\mathrm{d}w + \beta_{k+1}(y_{k+1}) \delta_{y_{k+1}}(A_{k+1})} \prod_{j=1,j\neq k+1}^n \delta_{y_j}(A_j)\right] \\
    &\qquad \left[\prod_{i=1}^k \left[\alpha_i(x_i, y_i)~\mathrm{d}y_i + \beta_i(x_i)~\delta_{x_i}(\mathrm{d}y_i)\right] \prod_{j=k+1}^n \delta_{x_j}(\mathrm{d}y_j)\right]
    \end{split} \\
    &= \left[\prod_{i=1}^{k+1}\paren{\int_{A_{i}} \alpha_{i}(y_{i}, w)~\mathrm{d}w + \beta_{i}(y_{i}) \delta_{x_{i}}(A_{i})}\right] \left[\prod_{j=k+2}^n \delta_{x_j}(A_j)\right].
\end{align}
This verifies that the composition kernel has the desired product structure. The special case of $k=n$ implies,
\begin{align}
    (K_n\circ\cdots\circ K_1)((x_1,\ldots, x_n), (\mathrm{d}y_1,\ldots,\mathrm{d}y_n)) = \prod_{i=1}^n \left[\alpha_i(x_i, y_i)~\mathrm{d}y_i + \beta_i(x_i)~\delta_{x_i}(\mathrm{d}y_i)\right].
\end{align}
To sample $(x_1',\ldots, x_n')\sim (K_n\circ\cdots\circ K_1)((x_1,\ldots, x_n), \cdot)$, one may simply sample independently from the distributions,
\begin{align}
    \mathrm{Pr}\left[x'_i \in A\vert x_i\right] = \int_{A} \alpha_i(x_i, w)~\mathrm{d}w + \beta_i(x_i) \delta_{x_i}(A)
\end{align}
for $i=1,\ldots, n$. Each of these samples may be drawn in parallel because the $i^\mathrm{th}$ sample depends only on $x_i$.


==> Adaptation of the Independent Metropolis-Hastings Sampler with Normalizing Flow Proposals/appendices/proof-concerning-deterministic-adaptations.tex <==
\clearpage
\section{Proofs Concerning Deterministic Adaptations}\label{app:proofs-concerning-deterministic-adaptations}


\begin{proposition}[\citet{roberts_rosenthal_2007}]\label{prop:deterministic-sequence-stationarity}
  Suppose that $(\theta_0,\theta_1,\ldots)$ is a {\it deterministic} $\mathcal{Y}$-valued sequence. Let $(K_{\theta_n})_{n\in\mathbb{N}}$ be an associated sequence of Markov transition kernels. If $\Pi$ is stationary for each $K_{\theta_n}$, then $\Pi$ is also the stationary distribution of the Markov chain whose transitions satisfy $X_{n+1}\sim K_{\theta_n}(X_n, \cdot)$.
\end{proposition}
\begin{proof}
Let $A\in\mathfrak{B}(\mathcal{X})$ and suppose $X_n\sim \Pi$. We will show $X_{n+1}\sim \Pi$.
\begin{align}
    \mathrm{Pr}\left[X_{n+1}\in A\right] &= \int_{\mathcal{X}} \mathrm{Pr}\left[X_{n+1}\in A\vert X_n=x\right] \cdot\mathrm{Pr}\left[X_n\in \mathrm{d}x\right] \\
    &= \int_{\mathcal{X}} \int_{\mathcal{Y}} \mathrm{Pr}\left[X_{n+1}\in A\vert X_n=x,\Theta_n=\theta\right] \cdot \delta_{\theta_n}(\mathrm{d}\theta) \cdot\mathrm{Pr}\left[X_n\in \mathrm{d}x\right] \\
    &= \int_{\mathcal{X}} K_{\theta_n}(x, A) \cdot\mathrm{Pr}\left[X_n\in \mathrm{d}x\right] \\
    &= \underset{x\sim \Pi}{\mathbb{E}}\left[K_{\theta_n}(x, A)\right] \\
    &= \Pi(A).
\end{align}
\end{proof}

\begin{lemma}\label{lem:transition-density-lower-bound}
For each $n\in\mathbb{N}$,
\begin{align}
    \label{eq:transition-density-lower-bound}K_{\theta_n}(x, \mathrm{d}x') \geq \frac{\pi_{\Pi}(x')}{M_{n}} \mu(\mathrm{d}x').
\end{align}
\end{lemma}
\begin{proof}
From \cref{eq:independent-metropolis-transition-kernel},
\begin{align}
    K_{\theta_n}(x, \mathrm{d}x') &\geq \min\set{1, \frac{\pi(x') \tilde{\pi}_{\theta_n}(x)}{\pi(x) \tilde{\pi}_{\theta_n}(x')}} ~\tilde{\pi}_{\theta_n}(x') ~\mu(\mathrm{d}x') \\
    &= \min\set{\tilde{\pi}_{\theta_n}(x'), \frac{\pi(x') \tilde{\pi}_{\theta_n}(x)}{\pi(x)}} ~\mu(\mathrm{d}x') \\
    &\geq \min\set{\tilde{\pi}_{\theta_n}(x'), \frac{\pi(x')}{M_{n}}} ~\mu(\mathrm{d}x') \\
    &= \frac{\pi(x')}{M_{n}}~\mu(\mathrm{d}x')
\end{align}
\end{proof}
\begin{corollary}\label{cor:small-state-space}
For any set $A\in\mathfrak{B}(\mathcal{X})$
\begin{align}
    K_{\theta_n}(x, A)\geq \frac{1}{M_{n}} \Pi(A).
\end{align}
\end{corollary}
\begin{proof}
Integrate both sides of \cref{eq:transition-density-lower-bound} over the set $A$.
\end{proof}

\begin{proof}[Proof of \Cref{thm:adaptive-total-variation-rate}]
From \cref{cor:small-state-space} it follows that we may express the transition kernel at step $n\in\mathbb{N}$ as
\begin{align}
    K_{\theta_n}(x, A) &= \frac{1}{M_{n}} \Pi(A) + \paren{1 - \frac{1}{M_{n}}} \cdot \underbrace{\frac{K_{\theta_n}(x, A) - \frac{1}{M_{n}}\Pi(A)}{1 - \frac{1}{M_{n}}}}_{\tilde{K}_{\theta_n}(x, A)} \\
    \label{eq:transition-mixture} &= \frac{1}{M_{n}} \Pi(A) + \paren{1 - \frac{1}{M_{n}}} \tilde{K}_{\theta_n}(x, A),
\end{align}
where $\tilde{K}_{\theta_n}(x, A)$ is another probability measure. With \cref{eq:transition-mixture}, $K_{\theta_n}$ may be given the following interpretation: With probability $1 / M_{n}$ generate the next state by the distribution $\Pi$ and with probability $1 - 1 / M_{n}$ generate the next state from the distribution $\tilde{K}_{\theta_n}$. Given an initial state $X_0=x_0$, consider the Markov chain whose transitions are generated according to $X_{n+1} \sim K_{\theta_n}(X_n, \cdot)$ with marginal laws $X_n\sim K^n(x_0, \cdot)$. From the representation in \cref{eq:transition-mixture} and \cref{prop:deterministic-sequence-stationarity}, it follows that the total variation distance is zero as soon as we generate the next state from $\Pi$. Let $T$ be the random variable representing the first step at which $X_{n}$ is generated from $\Pi$. Then $K^n(x_0, \cdot) = \mathrm{Pr}\left[T\leq n\right] \Pi(\cdot) + \mathrm{Pr}\left[T>n\right] \tilde{K}^n(x_0,\cdot)$, where $\tilde{K}^n$ is the mixture component of $K^n$ that is possibly not $\Pi$. Thus,
\begin{align}
    \Vert K^n(x_0, \cdot) - \Pi(\cdot)\Vert_{\mathrm{TV}} &=  \Vert \mathrm{Pr}\left[T\leq n\right] \Pi(\cdot) + \mathrm{Pr}\left[T>n\right] \tilde{K}^n(x_0,\cdot) - \Pi(\cdot)\Vert_{\mathrm{TV}} \\
    &= \Vert \mathrm{Pr}\left[T>n\right] \tilde{K}^n(x_0,\cdot) - \mathrm{Pr}\left[T>n\right]\Pi(\cdot)\Vert_{\mathrm{TV}} \\
    &= \mathrm{Pr}\left[T>n\right] \cdot\Vert \tilde{K}^n(x_0,\cdot) - \Pi(\cdot)\Vert_{\mathrm{TV}} \\
    &\leq 2\prod_{i=0}^{n-1} \paren{1 - \frac{1}{M_{i}}},
\end{align}
since $T>n$ only if we generate the next state from $\tilde{K}_{\theta_{i}}$ for $i=1,\ldots, n-1$, each of which occurs with probability $1 - 1 / M_{i}$.
\end{proof}

\begin{proposition}\label{prop:deterministic-sequence-non-increasing}
  Suppose that $(\theta_0,\theta_1,\ldots)$ is a {\it deterministic} $\mathcal{Y}$-valued sequence. Let $(K_{\theta_n})_{n\in\mathbb{N}}$ be an associated sequence of Markov transition kernels. If $\Pi$ is stationary for each $K_{\theta_n}$, then 
  \begin{align}
      \Vert K^{n+1}(x_0, \cdot) - \Pi(\cdot)\Vert_{\mathrm{TV}} \leq \Vert K^n(x_0, \cdot) -\Pi(\cdot)\Vert_{\mathrm{TV}},
  \end{align}
  where $K^n$ is defined in \cref{eq:deterministic-transition-law}.
\end{proposition}
\begin{proof}
\begin{align}
    \Vert K^{n+1}(x_0, \cdot) - \Pi(\cdot)\Vert_{\mathrm{TV}} &= \sup_{f\in\mathcal{M}} \abs{\int_{\mathcal{X}} f(y) K^{n+1}(x_0, \mathrm{d}y) - \int_{\mathcal{X}} f(y) \Pi(\mathrm{d}y)} \\
    &= \sup_{f\in\mathcal{M}} \abs{\int_{\mathcal{X}} f(y) K^{n+1}(x_0, \mathrm{d}y) - \int_{\mathcal{X}} f(y) \int_{\mathcal{X}} K_{\theta_n}(w, \mathrm{d}y) \Pi(\mathrm{d}w)} \\
    &= \sup_{f\in\mathcal{M}} \abs{\int_{\mathcal{X}} f(y) \int_{\mathcal{X}} K^{n}(x_0, \mathrm{d}w) K_{\theta_n}(w, \mathrm{d}y) - \int_{\mathcal{X}} f(y) \int_{\mathcal{X}} K_{\theta_n}(w, \mathrm{d}y) \Pi(\mathrm{d}w)} \\
    &= \sup_{f\in\mathcal{M}} \abs{\int_{\mathcal{X}} \paren{\int_{\mathcal{X}} f(y) K_{\theta_n}(w, \mathrm{d}y)}  K^{n}(x_0, \mathrm{d}w)  -  \int_{\mathcal{X}} \paren{\int_{\mathcal{X}} f(y) K_{\theta_n}(w, \mathrm{d}y)} \Pi(\mathrm{d}w)} \\
    &\leq \sup_{f\in\mathcal{M}} \abs{\int_{\mathcal{X}} f(w) K^n(x_0, \mathrm{d}w) - \int_{\mathcal{X}} f(w) \Pi(\mathrm{d}w)} \\
    &= \Vert K^n(x_0,\cdot) - \Pi(\cdot)\Vert_{\mathrm{TV}}.
\end{align}
\end{proof}
\begin{definition}\label{def:ergodic-set}
  Let $\Pi$ be a probability measure with density $\pi$. Suppose that every $\theta\in\mathcal{Y}$ parameterizes a probability measure $\tilde{\Pi}_\theta$ on $\mathfrak{B}(\mathcal{X})$ with density $\tilde{\pi}_{\theta}$. Define the ergodic set of $\Pi$ given $\mathcal{Y}$ as
  \begin{align}
      \mathcal{Q} = \set{\theta\in\mathcal{Y} : ~\text{there exists}~ M_\theta < \infty ~\text{such that} ~ \pi(x) \leq M_\theta \tilde{\pi}_\theta(x) ~~\forall~~ x\in\mathrm{Supp}(\pi)}.
  \end{align}
\end{definition}
The combination of \cref{prop:deterministic-sequence-non-increasing} and \cref{def:ergodic-set} allows one to give a slight generalization of \cref{thm:adaptive-total-variation-rate}.
\begin{corollary}\label{cor:deterministic-geometric-ergodicity}
Let $\Pi$ be a probability measure with density $\pi$. Suppose that every $\theta\in\mathcal{Y}$ parameterizes a probability measure $\tilde{\Pi}_\theta$ on $\mathfrak{B}(\mathcal{X})$ with density $\tilde{\pi}_{\theta}$. Suppose that $(\theta_0,\theta_1,\ldots)$ is a deterministic $\mathcal{Y}$-valued sequence. Let $(K_{\theta_n})_{n\in\mathbb{N}}$ be an associated sequence of Markov transition kernels of the independent Metropolis-Hastings sampler of $\Pi$ given $\tilde{\Pi}_{\theta_n}$. Let $K^n(x_0, A)$ denote the $n$-step transition probability from $x_0$ to $A\in\mathfrak{B}(\mathcal{X})$. Then
\begin{align}
    \Vert K^n(x_0,\cdot) - \Pi(\cdot)\Vert_{\mathrm{TV}} \leq 2\prod_{i=0}^{n-1} \paren{1 - L_i},
\end{align}
where
\begin{align}
    \label{eq:strong-doeblin-coefficient} L_i = \begin{cases}
    \frac{1}{M_i} & ~~\mathrm{if}~~ \theta_i \in\mathcal{Q} \\
    0 & ~~\mathrm{otherwise.}
    \end{cases}
\end{align}
\end{corollary}
\begin{proof}
The proof proceeds by induction. If $\theta_0 \in \mathcal{Q}$ then by argument in the proof of \cref{thm:adaptive-total-variation-rate} we have
\begin{align}
    \Vert K^1(x_0, \cdot) -\Pi(\cdot)\Vert_{\mathrm{TV}} &= \Vert K_{\theta_0}(x_0,\cdot) - \Pi(\cdot)\Vert_{\mathrm{TV}} \\
    &\leq 2 \paren{1 - \frac{1}{M_0}}.
\end{align}
If $\theta_0 \not\in Q$ then we obtain the vacuously true inequality $\Vert K^1(x_0, \cdot) -\Pi(\cdot)\Vert_{\mathrm{TV}}\leq 1$. Now assume that $\Vert K^n(x_0,\cdot)-\Pi(\cdot)\Vert_{\mathrm{TV}} \leq \prod_{i=0}^{n-1} (1 - L_i)$. If $\theta_n\not\in \mathcal{Q}$ then by \cref{prop:deterministic-sequence-non-increasing} we have
\begin{align}
    \Vert K^{n+1}(x_0,\cdot)-\Pi(\cdot)\Vert_{\mathrm{TV}} &\leq \Vert K^n(x_0,\cdot)-\Pi(\cdot)\Vert_{\mathrm{TV}} \\
    &\leq 2\prod_{i=0}^{n-1} (1 - L_i) \\
    &= 2\prod_{i=0}^{n-1} (1 - L_i) \cdot 1 \\
    &= 2\prod_{i=0}^{n} (1 - L_i),
\end{align}
since $L_n = 0$. On the other hand, if $\theta_n\in\mathcal{Q}$ then, using the same argument as in the proof of \cref{thm:adaptive-total-variation-rate}, the probability that none of $(X_0,\ldots,X_{n})$ were drawn from $\Pi$ is at most
\begin{align}
    \prod_{i=0}^{n-1} \paren{1 - L_i}.
\end{align}
Correspondingly, the probability that $X_{n+1}$ is also not drawn from $\Pi$ is $1 - 1/M_{n}$ so that the probability that none of $(X_0,\ldots, X_n, X_{n+1})$ is drawn from $\Pi$ is at most
\begin{align}
    \paren{1 - \frac{1}{M_n}}\prod_{i=0}^{n-1} \paren{1 - L_i} = \prod_{i=0}^n \paren{1 - L_i}.
\end{align}
From this the conclusion follows.
\end{proof}

==> Adaptation of the Independent Metropolis-Hastings Sampler with Normalizing Flow Proposals/appendices/proofs-concerning-compact-spaces.tex <==
\clearpage
\section{Proofs Concerning Simultaneous Uniform Ergodicity on Compact Spaces}\label{app:proofs-concerning-compact}

\begin{proof}[Proof of \Cref{cor:compact-uniformly-ergodic}]
  Because $\mathcal{X}$ is compact and $\pi$ and $\tilde{\pi}$ are continuous, we know that $\pi$ and $\tilde{\pi}$ attain maximum and minimum values on $\mathcal{X}$. Therefore, the ratio $\pi(x) / \tilde{\pi}(x)$ (i) does not diverge on $\mathrm{Supp}(\pi)$ because $\mathrm{Supp}(\pi)\subseteq \mathrm{Supp}(\tilde{\pi})$ and (ii) is bounded by
  \begin{align}
    \label{eq:upper-bound-ergodicity-constant} \frac{\max_{x\in\mathcal{X}} \pi(x)}{\min_{x\in\mathcal{X}} \tilde{\pi}(x)},
  \end{align}
  and $M$ is at most this value, with equality if the maximum of $\pi$ and the minimum of $\tilde{\pi}$ occur at the same point in $\mathcal{X}$.
\end{proof}


\begin{proof}[Proof of \Cref{prop:adaptive-simultaneous-ergodicity}]
  Define
  \begin{align}
      M_\theta = \max_{x\in\mathrm{Supp}(\pi)} \frac{\pi(x)}{\tilde{\pi}_{\theta}(x)}
  \end{align}
  and recall from \cref{cor:compact-uniformly-ergodic} that
  \begin{align}
    \Vert K_\theta^n(x,\cdot) - \pi\Vert_{\mathrm{TV}} \leq \paren{1 - \frac{1}{M_\theta}}^n.
  \end{align}
  From \cref{eq:upper-bound-ergodicity-constant} and \cref{eq:minimum-probability-density}, $M_\theta$ is bounded as
  \begin{align}
      M_\theta \leq  \frac{\max_{x\in\mathrm{Supp}(\pi)} \pi(x)}{\min_{x\in\mathrm{Supp}(\pi)}\tilde{\pi}_{\theta}(x)} \leq \frac{\max_{x\in\mathrm{Supp}(\pi)} \pi(x)}{\delta} = M_\delta
  \end{align}
  The quantity $M_\delta$ does not depend on $\theta\in\mathcal{Y}$ and therefore we have, for all $\theta\in\mathcal{Y}$,
  \begin{align}
    \Vert K_\theta^n(x,\cdot) - \pi\Vert_{\mathrm{TV}} \leq \paren{1 - \frac{1}{M_\delta}}^n.
  \end{align}
  Using this worst-case bound, we may find an $n$ satisfying \cref{def:simultaneous-uniform-ergodicity} for all $\theta\in\mathcal{Y}$.
\end{proof}

\begin{proof}[Proof of \Cref{lem:mixture-proposal-density}]
Fix $\theta\in\mathcal{Y}$. Then
\begin{align}
    \min_{x\in\mathrm{Supp}(\pi)} \tilde{\pi}^*_{\theta}(x) &= \min_{x\in\mathrm{Supp}(\pi)} \paren{\beta \pi^*_{\Pi^*}(x) + (1-\alpha) \tilde{\pi}_{\theta}(x)} \\
    &\geq \min_{x\in\mathrm{Supp}(\pi)} \beta \pi^*_{\Pi^*}(x) \\
    &= \delta.
\end{align}
The quantity $\delta$ is greater than zero since $\beta > 0$ and $\mathrm{Supp}(\pi)\subseteq \mathrm{Supp}(\pi^*_{\Pi^*})$. Since $\theta$ was arbitrary, the conclusion follows.
\end{proof}


==> Adaptation of the Independent Metropolis-Hastings Sampler with Normalizing Flow Proposals/appendices/proofs-concerning-containment.tex <==
\clearpage
\section{Proofs Concerning Containment}\label{app:proofs-concerning-containment}

\begin{proof}[Proof of \Cref{prop:containment-log-density}]
  \begin{align}
      & \mathrm{Pr}\left[\log \pi(x) - \log\tilde{\pi}_{\Theta_n}(x) < \log M~~\forall~~x\in\mathcal{X}\right] \geq 1-\delta~~\forall~~n\in\mathbb{N} \\
      \implies &\mathrm{Pr}\left[\frac{\pi(x)}{\tilde{\pi}_{\Theta_n}(x)} <  M~~\forall~~x\in\mathcal{X}\right] \geq 1-\delta~~\forall~~n\in\mathbb{N}
  \end{align}
  Then for all $\epsilon > 0$ there exists $N\equiv N(\epsilon, \delta)\in\mathbb{N}$ such that for all $x\in\mathcal{X}$,
  \begin{align}
      &\mathrm{Pr}\left[\Vert K_{\Theta_n}^N(x,\cdot) - \Pi(\cdot)\Vert_{\mathrm{TV}} <\epsilon\right]\geq 1-\delta ~~\forall~~n\in\mathbb{N}\\
      \implies& \mathrm{Pr}\left[W_\epsilon(x, K_{\Theta_n}) \leq N\right] \geq 1-\delta ~~\forall~~n\in\mathbb{N}.
  \end{align}
\end{proof}


==> Adaptation of the Independent Metropolis-Hastings Sampler with Normalizing Flow Proposals/appendices/proofs-concerning-continuity.tex <==
\clearpage
\section{Proofs Concerning Continuity of Independent Metropolis-Hastings Transition Kernels}\label{app:proofs-concerning-continuity}

% We first recall the bounded convergence theorem.
% \begin{theorem}
%   Let $(\mathcal{X}, \mathfrak{B}(\mathcal{X}), \mu)$ be a measure space with $\mu(\mathcal{X}) < \infty$. Let $f_n$ be a sequence of uniformly bounded $\mathbb{R}$-valued functions which converge pointwise to the function $f$. Then
%   \begin{align}
%       \lim_{n\to\infty} \int_{\mathcal{X}} f_n(x)~\mu(\mathrm{d}x) = \int_{\mathcal{X}} f(x)~\mu(\mathrm{d}x),
%   \end{align}
%   i.e. the mapping $f\mapsto \int_{\mathcal{X}} f(x) ~\mu(\mathrm{d}x)$ is continuous.
% \end{theorem}

\begin{theorem}\label{thm:continuous-mapping-theorem}
  Let $f$ be a continuous function from the metric space $(\mathcal{X}, d_{\mathcal{X}})$ to the metric space $(\mathcal{Y},d_{\mathcal{Y}})$. If $(X_0, X_1, \ldots)$ is a sequence of $\mathcal{X}$-valued random variables converging in probability to the random variable $X$ then $(f(X_0), f(X_1),\ldots)$ is a sequence of $\mathcal{Y}$-valued converging in probability to $f(X)$.
\end{theorem}

\begin{proof}[Proof of \Cref{lem:convergence-diminishing-adaptation}]
Given that $\theta\mapsto K_{\theta}$ is continuous, if $(\Theta_0,\Theta_1,\ldots)$ converges in probability to $\Theta$, we have immediately from \cref{thm:continuous-mapping-theorem} that $(K_{\Theta_0},K_{\Theta_1},\ldots)$ converges in probability to $K_{\Theta}$. This means that for all $\epsilon>0$ and $\delta>0$, there exists $N(\epsilon,\delta)\in\mathbb{N}$ such that $\mathrm{Pr}\left[d(K_{\Theta_n}, K_{\Theta}) < \epsilon\right] \geq 1-\delta$ for every $n\geq N$. For fixed $\epsilon > 0$ and $\delta > 0$, set $n \geq N(\epsilon/2, \delta)$ so that $\mathrm{Pr}\left[d(K_{\Theta_n}, K_{\Theta}) < \epsilon/2\right]\geq 1-\delta$. Thus,
\begin{align}
    \mathrm{Pr}\left[d(K_{\Theta_n}, K_{\Theta_{n+1}}) < \epsilon\right] &\geq \mathrm{Pr}\left[d(K_{\Theta_n}, K_{\Theta}) + d(K_{\Theta_{n+1}}, K_{\Theta} < \epsilon)\right] \\
    &\geq \mathrm{Pr}\left[d(K_{\Theta_n}, K_{\Theta}) < \epsilon / 2 ~\mathrm{and}~ d(K_{\Theta_{n+1}}, K_{\Theta}) < \epsilon / 2\right] \\
    &\geq \mathrm{Pr}\left[d(K_{\Theta_n}, K_{\Theta}) < \epsilon / 2\right] + \mathrm{Pr}\left[d(K_{\Theta_{n+1}}, K_{\Theta}) < \epsilon / 2\right] - 1 \\
    &\geq 1 - \delta + 1 - \delta - 1 \\
    &= 1 - 2\delta.
\end{align}
This establishes diminishing adaptation in the sense of \cref{def:diminishing-adaptation}.
\end{proof}

\begin{proof}[Proof of \Cref{prop:transition-kernel-distance}]
  To prove symmetry we write,
  \begin{align}
    d(K, K') &= \sup_{x\in\mathcal{X}} \Vert K(x, \cdot) - K'(x, \cdot)\Vert_{\mathrm{TV}} \\
    &= \sup_{x\in\mathcal{X}} \Vert K'(x, \cdot) - K(x, \cdot)\Vert_{\mathrm{TV}} \\
    &= d(K', K).
  \end{align}
  Identifiability follows from the definition of equality of Markov chain kernels given in \cref{def:transition-kernel-equality}. The triangle inequality is then proven as follows. Let $K''$ be another transition kernel on $\mathcal{X}\times\mathfrak{B}(\mathcal{X})$.
  \begin{align}
    d(K, K') &= \sup_{x\in\mathcal{X}} \Vert K(x, \cdot) - K'(x, \cdot)\Vert_{\mathrm{TV}} \\
    &\leq \sup_{x\in\mathcal{X}} \paren{\Vert K(x, \cdot) - K''(x, \cdot)\Vert_{\mathrm{TV}} + \Vert K''(x,\cdot) - K'(x,\cdot)\Vert_{\mathrm{TV}}} \\
    &\leq \sup_{x\in\mathcal{X}} \Vert K(x, \cdot) - K''(x, \cdot)\Vert_{\mathrm{TV}} + \sup_{x\in\mathcal{X}}\Vert K''(x,\cdot) - K'(x,\cdot)\Vert_{\mathrm{TV}} \\
    &= d(K, K'') + d(K'', K').
  \end{align}
\end{proof}

In the sequel, we will limit our discussion to the transition kernel of the independent Metropolis-Hastings sampler. Recall that this transition kernel has the following form,
\begin{align}
    K_{\theta}(x, A) = \int_A \alpha_{\theta}(x, y)\tilde{\pi}_{\theta}(y)~\mu(\mathrm{d}y) + \paren{1 - \int_{\mathcal{X}} \alpha_{\theta}(x, w)\tilde{\pi}_{\theta}(w) ~\mu(\mathrm{d}w)}\mathbf{1}\set{x\in A},
\end{align}
where
\begin{align}
    \alpha_{\theta}(x, y) = \min\set{1, \frac{\pi(y)\tilde{\pi}_{\theta}(x)}{\pi(x)\tilde{\pi}_{\theta}(y)}}.
\end{align}

\begin{lemma}\label{lem:convergence-independent-metropolis-hastings}
  Let $(\theta_1,\theta_2,\ldots)$ be a $\mathcal{Y}$-valued sequence converging to $\theta$. If for all $x\in\mathcal{X}$ and $A\in\mathfrak{B}(\mathcal{X})$ we have 
  \begin{align}
      \lim_{n\to\infty} \int_A \alpha_{\theta_n}(x, y) \tilde{\pi}_{\theta_n}(y)~\mu(\mathrm{d}y) &= \int_A \lim_{n\to\infty}\left[\alpha_{\theta_n}(x, y) \tilde{\pi}_{\theta_n}(y)\right] ~\mu(\mathrm{d}y) \\
      &= \int_A \alpha_{\theta}(x, y) \tilde{\pi}_{\theta}(y) ~\mu(\mathrm{d}y).
  \end{align}
%   \begin{enumerate}
%       \item \begin{align}
%           \lim_{n\to\infty} \alpha_{\theta_n}(x, y) \tilde{\pi}_{\theta_n}(y) = \alpha_{\theta}(x, y) \tilde{\pi}_{\theta}(y) 
%       \end{align}
%       \item \begin{align}
%           \lim_{n\to\infty} \int_A \alpha_{\theta_n}(x, y) \tilde{\pi}_{\theta_n}(y)~\mu(\mathrm{d}y) = \int_A \lim_{n\to\infty}\left[\alpha_{\theta_n}(x, y) \tilde{\pi}_{\theta_n}(y)\right] ~\mu(\mathrm{d}y)
%       \end{align}
%   \end{enumerate}
  then $\lim_{n\to\infty} K_{\theta_n} = K_\theta$.
  % $\lim_{n\to\infty} K_{\theta_n}(x, A) = K_{\theta}(x, A)$ then $\lim_{n\to\infty} K_{\theta_n} = K_\theta$.
\end{lemma}
\begin{proof}
By continuity of the distance function,
\begin{align}
    \lim_{n\to\infty} d(K_{\theta_n}, K_\theta) &= d(\lim_{n\to\infty} K_{\theta_n}, K_\theta) \\
    &= \sup_{x\in\mathcal{X}} \sup_{A\in\mathfrak{B}(\mathcal{X})} \abs{\lim_{n\to\infty} K_{\theta_n}(x, A) - K_\theta(x, A)}.
\end{align}
% which equals zero if $\lim_{n\to\infty} K_{\theta_n}(x, A) = K_\theta(x, A)$ for all $x\in\mathcal{X}$ and $A\in\mathfrak{B}(\mathcal{X})$.
Therefore,
\begin{align}
    \lim_{n\to\infty} K_{\theta_n}(x, A) &= \lim_{n\to\infty}\paren{\int_A \alpha_{\theta_n}(x, y)\tilde{\pi}_{\theta_n}(y)~\mu(\mathrm{d}y) + \paren{1 - \int_{\mathcal{X}} \alpha_{\theta_n}(x, w)\tilde{\pi}_{\theta_n}(w) ~\mu(\mathrm{d}w)}\mathbf{1}\set{x\in A}} \\
    &= \lim_{n\to\infty} \int_A \alpha_{\theta_n}(x, y)\tilde{\pi}_{\theta_n}(y)~\mu(\mathrm{d}y) + \lim_{n\to\infty} \paren{1 - \int_{\mathcal{X}} \alpha_{\theta_n}(x, w)\tilde{\pi}_{\theta_n}(w) ~\mu(\mathrm{d}w)}\mathbf{1}\set{x\in A} \\
    &= \int_A \lim_{n\to\infty} \left[\alpha_{\theta_n}(x, y)\tilde{\pi}_{\theta_n}(y)\right]~\mu(\mathrm{d}y) + \paren{1 - \int_{\mathcal{X}} \lim_{n\to\infty}\left[\alpha_{\theta_n}(x, w)\tilde{\pi}_{\theta_n}(w)\right] ~\mu(\mathrm{d}w)}\mathbf{1}\set{x\in A} \\
    &= \int_A \alpha_{\theta}(x, y)\tilde{\pi}_{\theta}(y)~\mu(\mathrm{d}y) + \paren{1 - \int_{\mathcal{X}} \alpha_{\theta}(x, w)\tilde{\pi}_{\theta}(w) ~\mu(\mathrm{d}w)}\mathbf{1}\set{x\in A} \\
    &= K_{\theta}(x, A).
\end{align}
Finally,
\begin{align}
    \lim_{n\to\infty} d(K_{\theta_n}, K_\theta) &= \sup_{x\in\mathcal{X}} \sup_{A\in\mathfrak{B}(\mathcal{X})} \abs{\lim_{n\to\infty} K_{\theta_n}(x, A) - K_\theta(x, A)} \\
    &= \sup_{x\in\mathcal{X}} \sup_{A\in\mathfrak{B}(\mathcal{X})} \abs{K_{\theta}(x, A) - K_\theta(x, A)} \\
    &= 0.
\end{align}
\end{proof}

The following result is called Scheff\'{e}'s lemma; see \citet{lebanon-probability,pollard_2001}.
\begin{lemma}\label{lem:scheffes-lemma}
  Let $\pi_n$ be a sequence of probability densities that converge pointwise to another density $\pi$. Then, let $\Pi(A) = \int_A \pi(x)~\mu(\mathrm{d}x)$ and $\Pi_n(A) = \int_A \pi_n(x)~\mu(\mathrm{d}x)$ be the measures whose densities are $\pi$ and $\pi_n$ with respect to dominating measure $\mu$, respectively. Then $\lim_{n\to\infty}\Vert \Pi(\cdot) - \Pi_n(\cdot)\Vert_{\mathrm{TV}} = 0$.
\end{lemma}
We will also require the following theorem from \citet[Page 270]{alma991018098349703276}.
\begin{theorem}\label{thm:variable-measure-dominated-convergence}
  Let $(\mathcal{X},\mathfrak{B}(\mathcal{X}))$ be a measurable space and let $(\Pi_n)_{n\in\mathbb{N}}$ be a sequence of probability measures converging to the probability measure $\Pi$. Let $\alpha_n: \mathcal{X}\to\R$ and $\beta_n : \mathcal{X}\to\R$ be two sequences of functions converging pointwise to the functions $\alpha$ and $\beta$, respectively. Suppose further that $\abs{\alpha_n(x)} \leq \beta_n(x)$ for every $x\in\mathcal{X}$ and that,
  \begin{align}
      \lim_{n\to\infty} \int_{\mathcal{X}} \beta_n(x) ~\Pi_n(\mathrm{d}x) = \int_{\mathcal{X}} \beta(x)~\Pi(\mathrm{d}x) < \infty.
  \end{align}
  Then,
  \begin{align}
      \lim_{n\to\infty} \int_{A} \alpha_n(x)~\Pi_n(\mathrm{d}x) = \int_A \alpha(x) ~\Pi(\mathrm{d}x), 
  \end{align}
  for $A\in\mathfrak{B}(\mathcal{X})$
\end{theorem}

\begin{lemma}\label{lem:continuous-pointwise}
  Suppose that for fixed $x\in\mathcal{X}$ the mapping $\theta\mapsto \tilde{\pi}_{\theta}(x)$ is continuous, that $y\in \mathcal{X}$, and that $\mathrm{Supp}(\tilde{\pi}_\theta) = \mathcal{X}$ for every $\theta\in\mathcal{Y}$. Let $(\theta_1,\theta_2,\ldots)$ be a $\mathcal{Y}$-valued sequence converging to $\theta$. Then $\lim_{n\to\infty} \alpha_{\theta_n}(x, y)\tilde{\pi}_{\theta_n}(y) =\alpha_{\theta}(x, y)\tilde{\pi}_{\theta}(y)$ pointwise.
\end{lemma}
\begin{proof}
\begin{align}
    \lim_{n\to\infty} \alpha_{\theta_n}(x, y) &= \lim_{n\to\infty} \min\set{1, \frac{\pi(y)\tilde{\pi}_{\theta_n}(x)}{\pi(x)\tilde{\pi}_{\theta_n}(y)}} \\
    &= \paren{\lim_{n\to\infty} \min\set{1, \frac{\pi(y)\tilde{\pi}_{\theta_n}(x)}{\pi(x)\tilde{\pi}_{\theta_n}(y)}}} \\
    &= \paren{\lim_{n\to\infty} \min\set{1, \frac{\pi(y)\tilde{\pi}_{\theta_n}(x)}{\pi(x)\tilde{\pi}_{\theta_n}(y)}}} \\
    &= \paren{ \min\set{1, \lim_{n\to\infty} \frac{\pi(y)\tilde{\pi}_{\theta_n}(x)}{\pi(x)\tilde{\pi}_{\theta_n}(y)}}} \\
    &= \paren{ \min\set{1, \frac{\pi(y)}{\pi(x)}\lim_{n\to\infty} \frac{\tilde{\pi}_{\theta_n}(x)}{\tilde{\pi}_{\theta_n}(y)}}} \\
    &= \paren{ \min\set{1, \frac{\pi(y)}{\pi(x)}\paren{\lim_{n\to\infty} \tilde{\pi}_{\theta_n}(x)} \paren{\lim_{n\to\infty} \frac{1}{\tilde{\pi}_{\theta_n}(y)}}}} \\
    \label{eq:continuity-full-support} &= \paren{ \min\set{1, \frac{\pi(y)}{\pi(x)}\paren{ \tilde{\pi}_{\theta}(x)} \paren{ \frac{1}{\lim_{n\to\infty} \tilde{\pi}_{\theta_n}(y)}}}} \\
    &= \paren{ \min\set{1, \frac{\pi(y)}{\pi(x)}\paren{ \tilde{\pi}_{\theta}(x)} \paren{ \frac{1}{ \tilde{\pi}_{\theta}(y)}}}} \\
    &= \alpha_{\theta}(x, y).
\end{align}
The assumption that $\mathrm{Supp}(\tilde{\pi}_\theta) = \mathcal{X}$ is used in \cref{eq:continuity-full-support}.
\end{proof}

\begin{corollary}\label{cor:variable-measure-bounded-convergence}
  Let $(\theta_1,\theta_2,\ldots)$ be a $\mathcal{Y}$-valued sequence converging to $\theta$.  Let $\pi$ be a probability density function on a compact space $\mathcal{X}$ and let $\tilde{\pi}_{\theta}$ be a family of density functions on $\mathcal{X}$ indexed by $\theta$ such that the map $\theta\mapsto \tilde{\pi}_{\theta}$ is continuous (i.e. $\pi_{\theta_n}\to \pi_{\theta}$). Assume further that $\mathrm{Supp}(\tilde{\pi}_\theta) = \mathcal{X}$ for every $\theta\in\mathcal{Y}$.
  Let $x\in\mathcal{X}$ be fixed and let $y\in\mathcal{X}$. Define
  \begin{align}
      \alpha_{\theta}(x, y) = \min\set{1, \frac{\pi(y)\tilde{\pi}_{\theta}(x)}{\pi(x)\tilde{\pi}_{\theta}(y)}}.
  \end{align}
  Then,
  \begin{align}
      \lim_{n\to\infty} \int_A \alpha_{\theta_n}(x, y) \tilde{\pi}_{\theta_n}(y)~\mu(\mathrm{d}y) = \int_A \alpha_{\theta}(x, y) \tilde{\pi}_{\theta}(y)~\mu(\mathrm{d}y)
  \end{align}
\end{corollary}
\begin{proof}
This follows immediate from \cref{thm:variable-measure-dominated-convergence} with $\beta_n(x) \equiv 1$ and the measures $\Pi_n(A) = \int_A \tilde{\pi}_{\theta_n}(x)~\mu(\mathrm{d}x)$ and $\Pi(A) = \int_A \tilde{\pi}_{\theta}(x)~\mu(\mathrm{d}x)$, which converge by \cref{lem:scheffes-lemma}.
\end{proof}

% \begin{corollary}
%   Let $(\theta_1,\theta_2,\ldots)$ be a $\mathcal{Y}$-valued sequence converging to $\theta$. Let $\pi$ be a probability density function on a compact space $\mathcal{X}$ and let $\tilde{\pi}_{\theta}$ be a family of density functions on $\mathcal{X}$ indexed by $\theta$. Suppose further that $\tilde{\pi}_{\theta}$ are uniformly bounded; that is, there exists $L\in\mathbb{R}_+$ such that $\tilde{\pi}_{\theta}(x) \leq L$ for all $x\in\mathcal{X}$ and $\theta\in\mathcal{Y}$. For $x$ and $y$ in $\mathcal{X}$, define
%   \begin{align}
%       \alpha_{\theta}(x, y) = \min\set{1, \frac{\pi(y)\tilde{\pi}_{\theta}(x)}{\pi(x)\tilde{\pi}_{\theta}(y)}}.
%   \end{align}
%   Let $A\in\mathfrak{B}(\mathcal{X})$. Then, if $\lim_{n\to\infty} \alpha_{\theta_n}(x, y)\tilde{\pi}_{\theta_n}(y) =\alpha_{\theta}(x, y)\tilde{\pi}_{\theta}(y)$ pointwise, the mapping
%   \begin{align}
%       \theta\mapsto \int_{A} \alpha_{\theta}(x, y)\tilde{\pi}_{\theta}(y) ~\mu(\mathrm{d}y)
%   \end{align}
%   is continuous for fixed $x$.
% \end{corollary}
% \begin{proof}
% This follows immediately from the bounded convergence theorem and noting that $\alpha_{\theta}(x, y)\tilde{\pi}_{\theta}(y)$ is uniformly bounded by $L$. Since $\mathcal{X}$ is compact and $A\subset \mathcal{X}$, the integrable function $g(x) = L$ suffices to give the result.
% \end{proof}




\begin{proof}[Proof of \cref{thm:continuity-parameterization}]
Fix $x\in\mathcal{X}$ and $A\in\mathfrak{B}(\mathcal{X})$. Thus,
\begin{align}
    \lim_{n\to\infty} K_{\theta_n}(x, A) &= \lim_{n\to\infty}\paren{\int_A \alpha_{\theta_n}(x, y)\tilde{\pi}_{\theta_n}(y)~\mu(\mathrm{d}y) + \paren{1 - \int_{\mathcal{X}} \alpha_{\theta_n}(x, w)\tilde{\pi}_{\theta_n}(w) ~\mu(\mathrm{d}w)}\mathbf{1}\set{x\in A}} \\
    &= \lim_{n\to\infty} \int_A \alpha_{\theta_n}(x, y)\tilde{\pi}_{\theta_n}(y)~\mu(\mathrm{d}y) + \lim_{n\to\infty} \paren{1 - \int_{\mathcal{X}} \alpha_{\theta_n}(x, w)\tilde{\pi}_{\theta_n}(w) ~\mu(\mathrm{d}w)}\mathbf{1}\set{x\in A} \\
    \label{eq:interchange-limits} &= \int_A \alpha_{\theta}(x, y)\tilde{\pi}_{\theta}(y)~\mu(\mathrm{d}y) + \paren{1 - \int_{\mathcal{X}} \alpha_{\theta}(x, w)\tilde{\pi}_{\theta}(w) ~\mu(\mathrm{d}w)}\mathbf{1}\set{x\in A} \\
    &= K_{\theta}(x, A).
\end{align}
where we have used \cref{cor:variable-measure-bounded-convergence} in \cref{eq:interchange-limits}. The conclusion then follows from \cref{lem:convergence-independent-metropolis-hastings}.
\end{proof}

% \begin{proof}[Proof of \cref{thm:continuity-parameterization}]
% Fix $x\in\mathcal{X}$ and $A\in\mathfrak{B}(\mathcal{X})$. The transition kernel of the independent Metropolis-Hastings sampler can be written as,
% \begin{align}
%     K_{\theta_n}(x, A) = \int_A \alpha_{\theta_n}(x, y)\tilde{\pi}_{\theta_n}(y)~\mu(\mathrm{d}y) + \paren{1 - \int_{\mathcal{X}} \alpha_{\theta_n}(x, w)\tilde{\pi}_{\theta_n}(w) ~\mu(\mathrm{d}w)}\mathbf{1}\set{x\in A}.
% \end{align}
% Thus,
% \begin{align}
%     \lim_{n\to\infty} K_{\theta_n}(x, A) &= \lim_{n\to\infty}\paren{\int_A \alpha_{\theta_n}(x, y)\tilde{\pi}_{\theta_n}(y)~\mu(\mathrm{d}y) + \paren{1 - \int_{\mathcal{X}} \alpha_{\theta_n}(x, w)\tilde{\pi}_{\theta_n}(w) ~\mu(\mathrm{d}w)}\mathbf{1}\set{x\in A}} \\
%     &= \lim_{n\to\infty} \int_A \alpha_{\theta_n}(x, y)\tilde{\pi}_{\theta_n}(y)~\mu(\mathrm{d}y) + \lim_{n\to\infty} \paren{1 - \int_{\mathcal{X}} \alpha_{\theta_n}(x, w)\tilde{\pi}_{\theta_n}(w) ~\mu(\mathrm{d}w)}\mathbf{1}\set{x\in A} \\
%     &= \int_A \alpha_{\theta}(x, y)\tilde{\pi}_{\theta}(y)~\mu(\mathrm{d}y) + \paren{1 - \int_{\mathcal{X}} \alpha_{\theta}(x, w)\tilde{\pi}_{\theta}(w) ~\mu(\mathrm{d}w)}\mathbf{1}\set{x\in A} \\
%     &= K_{\theta}(x, A).
% \end{align}
% Since $x\in\mathcal{X}$ and $A\in\mathfrak{B}(\mathcal{X})$ were arbitrary, this establishes $\lim_{n\to\infty} d(K_{\theta_n}, K_\theta) = 0$ from which it follows $\lim_{n\to\infty} K_{\theta_n} = K_\theta$; that is the mapping $\theta\mapsto K_\theta$ is continuous.
% \end{proof}


==> Adaptation of the Independent Metropolis-Hastings Sampler with Normalizing Flow Proposals/appendices/proofs-concerning-independent-adaptations.tex <==
\clearpage
\section{Proofs Concerning Independent Adaptations}\label{app:proofs-concerning-independent-adaptations}

\begin{theorem}\label{thm:total-variation-rate-independent-adaption}
Let $\Pi$ be a probability measure with density $\pi$. Suppose that every $\theta\in\mathcal{Y}$ parameterizes a probability measure $\tilde{\Pi}_\theta$ on $\mathfrak{B}(\mathcal{X})$ with density $\tilde{\pi}_{\theta}$. Suppose that $(\Theta_0,\Theta_1,\ldots)$ is a {\it stochastic} $\mathcal{Y}$-valued sequence. Let $(K_{\Theta_n})_{n\in\mathbb{N}}$ be an associated sequence of Markov transition kernels of the independent Metropolis-Hastings sampler of $\Pi$ given $\tilde{\Pi}_{\Theta_n}$. Suppose that $X_n$ and $\Theta_n$ are independent given the history of the chain to step $n-1$. Let $G^n(x_0, A)$ be the associated marginal transition law. Then
\begin{align}
    \Vert G^n(x_0, \cdot) - \Pi(\cdot)\Vert_{\mathrm{TV}} \leq 2\underset{(\Theta_0,\ldots,\Theta_{n-1})}{\mathbb{E}} \left[\prod_{i=0}^{n-1} \paren{1 - L_i}\right]
\end{align}
where $L_i=1/M_i$ if $M_i<\infty$ and otherwise $L_i=0$.
\end{theorem}
A proof is given in \cref{app:proofs-concerning-independent-adaptations}. This result was previously demonstrated in \citet{adaptive-independent-metropolis}, though we have offered a different proof procedure.
\begin{example}\label{ex:normalizing-flow-stochastic}
Let $\Pi$ be a probability measure with density $\pi$. Let $\mathcal{Y}=\R^m$ and suppose that every $\theta\in\mathcal{Y}$ smoothly parameterizes a probability measure $\tilde{\Pi}$ on $\mathfrak{B}(\mathcal{X})$ with density $\tilde{\pi}_{\theta}$ for which $\mathrm{Supp}(\pi)= \mathrm{Supp}(\tilde{\pi}_{\theta})$. Consider the sequence of updates,
\begin{align}
  \label{eq:gd-rev-kl}
  \theta_{n} &= \theta_{n-1} - \epsilon \nabla_\theta \left(\frac{1}{s}\sum_{i=1}^s \log \frac{\tilde{\pi}_{\theta_{n-1}}(Y_s(\theta_{n-1}))}{\pi(Y_s(\theta_{n-1}))}\right)
\end{align}
where $Y_1,\ldots,Y_s\overset{\mathrm{i.i.d.}}{\sim} \tilde{\Pi}_{\theta_{n-1}}$. This corresponds to the stochastic gradient approximation of \cref{ex:exact-flow}.
Consider the family of Markov chain transition operators of the independent Metropolis-Hastings sampler of $\Pi$ given $\tilde{\Pi}_{\theta_n}$ with transition kernels $K_{\theta_n}$. Then $\Pi$ is the stationary distribution of the Markov chain whose transitions satisfy $X_{n+1}\sim K_{\theta_n}(X_n, \cdot)$. To see this, let $\tilde{X}$ be a sample from $\tilde{\Pi}_{\theta_{n-1}}$ independent of $(Y_1,\ldots,Y_s)$ and let $U\sim\mathrm{Uniform}(0, 1)$ be independent of both. Then $X_{n} = g(x_{n-1}, \theta_{n-1}, \tilde{X}, U)$ where $g$ is given by,
\begin{align}
g(x, \theta, \tilde{x}, u) = \begin{cases}
\tilde{x} & ~~\mathrm{if}~~ u <\min\set{1, \frac{\pi(\tilde{x}) \tilde{\pi}_{\theta}(x)}{\pi(x) \tilde{\pi}_{\theta}(\tilde{x})}} \\
x & ~~\mathrm{otherwise}
\end{cases}
\end{align}
and $\Theta_n = f(\theta_{n-1}, Y_1,\ldots,Y_s)$ where $f$ is given by,
\begin{align}
    f(\theta, y_1(\theta),\ldots, y_s(\theta)) = \theta - \epsilon \nabla_\theta \left(\frac{1}{s}\sum_{i=1}^s \log \frac{\tilde{\pi}_{\theta}(y_s(\theta))}{\pi(y_s(\theta))}\right).
\end{align}
By \cref{lem:functions-of-independent-variables}, $\Theta_n$ and $X_n$ are independent given the history of the chain to step $n-1$ and therefore, by \cref{prop:stochastic-sequence-stationarity}, $\Pi$ is the stationary distribution.
\end{example}

\begin{lemma}\label{lem:functions-of-independent-variables}
Suppose that $(X_1^{(a)},\ldots, X_r^{(a)})$ and $(X_1^{(b)},\ldots,X_s^{(b)})$ are two sets of random variables which are independent given the history of the chain to step $n-1$. Suppose that $\Theta_n = f(x_{n-1}, \theta_{n-1}, X_1^{(a)},\ldots, X_r^{(a)})$ and $X_{n} = g(x_{n-1}, \theta_{n-1}, X_1^{(b)},\ldots,X_s^{(b)})$ for two functions $f$ and $g$. Then $X_n$ and $\Theta_n$ are independent given the history of the chain to step $n-1$.
\end{lemma}
\begin{proof}
The $\sigma$-algebra generated by $\Theta_n$ is a subset of the $\sigma$-algebra generated by $(X_1^{(a)},\ldots, X_r^{(a)})$. Likewise, the $\sigma$-algebra generated by $X_n$ is a subset of the $\sigma$-algebra generated by $(X_1^{(b)},\ldots,X_s^{(b)})$. Since $(X_1^{(a)},\ldots, X_r^{(a)})$ and $(X_1^{(b)},\ldots,X_s^{(b)})$ are assumed independent given the history of the chain to step $n-1$, the conclusion follows.
\end{proof}
\begin{proof}[Proof of \Cref{thm:total-variation-rate-independent-adaption}]
\begin{align}
    \Vert G^n(x_0, \cdot) - \Pi(\cdot)\Vert_{\mathrm{TV}} &= \Vert \underset{(\Theta_0,\ldots,\Theta_{n-1})}{\mathbb{E}} K^n_{(\Theta_0,\ldots,\Theta_{n-1})}(x_0, \cdot) - \Pi(\cdot)\Vert_{\mathrm{TV}} \\
    &= 2\sup_{A\in\mathfrak{B}(\mathcal{X})} \abs{\underset{(\Theta_0,\ldots,\Theta_{n-1})}{\mathbb{E}} K^n_{(\Theta_0,\ldots,\Theta_{n-1})}(x_0, A) - \Pi(A)} \\
    &\leq \underset{(\Theta_0,\ldots,\Theta_{n-1})}{\mathbb{E}} 2\sup_{A\in\mathfrak{B}(\mathcal{X})} \abs{ K^n_{(\Theta_0,\ldots,\Theta_{n-1})}(x_0, A) - \Pi(A)} \\
    &= \underset{(\Theta_0,\ldots,\Theta_{n-1})}{\mathbb{E}} \Vert K^n_{(\Theta_0,\ldots,\Theta_{n-1})}(x_0, \cdot) - \Pi(\cdot)\Vert_{\mathrm{TV}} \\
    &\leq 2\underset{(\Theta_0,\ldots,\Theta_{n-1})}{\mathbb{E}} \left[\prod_{i=0}^{n-1} \paren{1 - L_i}\right],
\end{align}
where the first inequality can be deduced as follows: By Jensen's inequality,
\begin{align}
    \abs{\underset{(\Theta_0,\ldots,\Theta_{n-1})}{\mathbb{E}} K^n_{(\Theta_0,\ldots,\Theta_{n-1})}(x_0, A) - \Pi(A)} \leq \underset{(\Theta_0,\ldots,\Theta_{n-1})}{\mathbb{E}} \abs{K^n_{(\Theta_0,\ldots,\Theta_{n-1})}(x_0, A) - \Pi(A)}.
\end{align}
Moreover,
\begin{align}
    &\abs{K^n_{(\Theta_0,\ldots,\Theta_{n-1})}(x_0, A) - \Pi(A)} \leq \sup_{A\in\mathfrak{B}(\mathcal{X})} \abs{K^n_{(\Theta_0,\ldots,\Theta_{n-1})}(x_0, A) - \Pi(A)} \\
    \implies& \underset{(\Theta_0,\ldots,\Theta_{n-1})}{\mathbb{E}} \abs{K^n_{(\Theta_0,\ldots,\Theta_{n-1})}(x_0, A) - \Pi(A)} \leq \underset{(\Theta_0,\ldots,\Theta_{n-1})}{\mathbb{E}} \sup_{A\in\mathfrak{B}(\mathcal{X})} \abs{K^n_{(\Theta_0,\ldots,\Theta_{n-1})}(x_0, A) - \Pi(A)} \\
    \implies& \sup_{A\in\mathfrak{B}(\mathcal{X})} \underset{(\Theta_0,\ldots,\Theta_{n-1})}{\mathbb{E}} \abs{K^n_{(\Theta_0,\ldots,\Theta_{n-1})}(x_0, A) - \Pi(A)} \leq \underset{(\Theta_0,\ldots,\Theta_{n-1})}{\mathbb{E}} \sup_{A\in\mathfrak{B}(\mathcal{X})} \abs{K^n_{(\Theta_0,\ldots,\Theta_{n-1})}(x_0, A) - \Pi(A)}
\end{align}
The second inequality follows from \cref{cor:deterministic-geometric-ergodicity} as follows:
\begin{align}
    &\Vert K^n_{(\Theta_0,\ldots,\Theta_{n-1})}(x_0, \cdot) - \Pi(\cdot)\Vert_{\mathrm{TV}} \leq 2\prod_{i=0}^{n-1} (1 - L_i) \\
    \implies& \underset{(\Theta_0,\ldots,\Theta_{n-1})}{\mathbb{E}} \Vert K^n_{(\Theta_0,\ldots,\Theta_{n-1})}(x_0, \cdot) - \Pi(\cdot)\Vert_{\mathrm{TV}} \leq 2\underset{(\Theta_0,\ldots,\Theta_{n-1})}{\mathbb{E}} \left[\prod_{i=0}^{n-1} (1 - L_i)\right].
\end{align}
\end{proof}


==> Adaptation of the Independent Metropolis-Hastings Sampler with Normalizing Flow Proposals/appendices/pseudo-likelihood-algorithm.tex <==
\clearpage
\section{Pseudo-Likelihood Algorithm}\label{app:pseudo-likelihood-algorithm}

\input{algorithms/independent-adaptive}


==> Adaptation of the Independent Metropolis-Hastings Sampler with Normalizing Flow Proposals/appendices/simultaneous-uniform-ergodicity-compact.tex <==
\clearpage
\section{Simultaneous Uniform Ergodicity on Compact Spaces}\label{app:simultaneous-uniform-ergodicity-compact}

\begin{definition}\label{def:simultaneous-uniform-ergodicity}
  A family of transition kernels $\set{K_\theta : \theta\in\mathcal{Y}}$ is said to exhibit simultaneous uniform ergodicity if, for all $\epsilon>0$, there exists $n\in \mathbb{N}$ such that $\Vert K_\theta^n(x,\cdot) - \Pi(\cdot)\Vert_{\mathrm{TV}} \leq \epsilon$ for all $\theta\in\mathcal{Y}$ and $x\in\mathcal{X}$.
\end{definition}
Simultaneous uniform ergodicity is a strong condition which states that, no matter which parameter $\theta\in\mathcal{Y}$ one selects, there is a finite number of steps one can take with that fixed transition kernel in order to become arbitrarily close to the target distribution in total variation. We will see later that this condition can be made to hold for compactly supported target distributions.

We now turn our attention to the question of simultaneous uniform ergodicity. 
\begin{proposition}\label{prop:adaptive-simultaneous-ergodicity}
  Let $\mathcal{X}$ and $\pi$ satisfy the conditions of \cref{cor:compact-uniformly-ergodic}. Suppose that every $\theta\in\mathcal{Y}$ parameterizes a probability measure $\tilde{\Pi}_\theta$ on $\mathfrak{B}(\mathcal{X})$ whose density $\tilde{\pi}_{\theta}$ is continuous and satisfies $\mathrm{Supp}(\pi)\subseteq \mathrm{Supp}(\tilde{\pi}_{\theta})$. Suppose further that for all $\theta\in\mathcal{Y}$, there exists $\delta > 0$ such that
  \begin{align}
    \label{eq:minimum-probability-density} \delta \leq \min_{x\in\mathrm{Supp}(\pi)} \tilde{\pi}_{\theta}(x)
  \end{align}
  Then the family of Markov chain transition operators of the independent Metropolis-Hastings sampler of $\Pi$ given $\tilde{\Pi}_\theta$ satisfies the simultaneous uniform ergodicity property.
\end{proposition}
A proof is given in \cref{app:proofs-concerning-compact}. Perhaps the most straight-forward mechanism to guarantee \cref{eq:minimum-probability-density} is to consider mixture distributions with a fixed distribution that shares the same support as $\pi$.
\begin{lemma}\label{lem:mixture-proposal-density}
  Suppose that $\Pi^*$ is a distribution on $\mathcal{X}$ with continuous density $\pi^*_{\Pi^*}$ such that $\mathrm{Supp}(\pi)\subseteq \mathrm{Supp}(\pi^*_{\Pi^*})$. Suppose that every $\theta\in\mathcal{Y}$ parameterizes a probability measure $\tilde{\Pi}_\theta$ on $\mathfrak{B}(\mathcal{X})$ whose density $\tilde{\pi}_{\theta}$ is continuous. Consider probability measures $\tilde{\Pi}_\theta^*$ whose densities are constructed from mixtures,
  \begin{align}
    \tilde{\pi}^*_{\theta}(x) = \beta \pi^*_{\Pi^*}(x) + (1-\beta) \tilde{\pi}_{\theta}(x),
  \end{align}
  where $\beta\in(0,1)$. Then $\tilde{\pi}^*_{\theta}$ satisfies \cref{eq:minimum-probability-density} with
  \begin{align}
      \label{eq:mixture-minimum-density} \delta = \beta \min_{x\in\mathrm{Supp}(\pi)} \pi^*_{\Pi^*}(x).
  \end{align}
\end{lemma}

A proof is given in \cref{app:proofs-concerning-compact}. A natural choice of $\Pi^*$ would be the uniform distribution on $\mathcal{X}$. It is conceivable that one could consider adapting $\beta$ in the same way that one adapts $\theta$. However, in order to guarantee that \cref{eq:mixture-minimum-density} is greater than zero, one will require the condition that $\beta \in (\beta_*, 1)$ where $\beta_* > 0$.

\begin{example}
  Let $\Pi$ be a probability measure with density $\pi$ on a compact space $\mathcal{X}$. Let $\mathcal{Y}=\R^m$ and suppose that every $\theta\in\mathcal{Y}$ smoothly parameterizes a probability measure $\tilde{\Pi}_\theta$ on $\mathfrak{B}(\mathcal{X})$ with density $\tilde{\pi}_{\theta}$ for which $\mathrm{Supp}(\pi)= \mathrm{Supp}(\tilde{\pi}_{\theta})$. Let $\tilde{\Pi}_{\theta}^*$ be as in \cref{lem:mixture-proposal-density}. Let $(\alpha_0,\alpha_1,\ldots)$ be a sequence, bounded between zero and one, converging to zero. Consider the sequence of updates,
\begin{align}
  \theta_{n} &= \begin{cases}\theta_{n-1} - \epsilon \nabla_\theta \log \frac{\tilde{\pi}_{\theta_{n-1}}(\tilde{X}(\theta_{n-1}))}{\pi(\tilde{X}(\theta_{n-1}))} &~~\mathrm{w.p.}~~ 1-\alpha_{n-1} \\
  \theta_{n-1} & ~~\mathrm{otherwise.}
  \end{cases}
\end{align}
where $\tilde{X}\sim \tilde{\Pi}_{\theta_{n-1}}^*$.
Consider the family of Markov chain transition operators of the independent Metropolis-Hastings sampler of $\Pi$ given $\tilde{\Pi}_{\theta_n}^*$ with transition kernels $K_{\theta_n}$ where the proposal at step $n$ is $\tilde{X}$. Then by \cref{thm:ergodic-diminishing-simultaneous} the distribution of $X_{n+1} \sim K_{\theta_n}(X_n, \cdot)$ converges to $\Pi$.
\end{example}

Examples of compact spaces on which normalizing flows have been applied include the torus, the sphere, the special orthogonal group, and the Stiefel manifold \citep{DBLP:conf/icml/RezendePRAKSC20,pmlr-v89-falorsi19a}.

The reason we were required to invoke a mixture distribution in the adaptation was because it prevented any sequence from becoming arbitrarily ill-suited to sampling the target distribution; the fact that there was a global limit to how bad any proposal distribution could be allowed us to invoke simultaneous uniform ergodicity of the family of distributions. 


==> Adaptation of the Independent Metropolis-Hastings Sampler with Normalizing Flow Proposals/appendices/total-variation-review.tex <==
\clearpage
\section{Review of Total Variation Distance}\label{app:total-variation-review}

Similarity of probability measures can be assessed with respect to several criteria. A ubiquitous notion of distance between probability measures is given by the total variation norm of their difference.
\begin{definition}\label{def:total-variation-norm}
Let $\nu_1$ and $\nu_2$ be probability measures on $(\mathcal{X},\mathfrak{B}(\mathcal{X}))$. Then the total variation distance between $\nu_1$ and $\nu_2$ is defined by,
\begin{align}
    \Vert \nu_1(\cdot)-\nu_2(\cdot)\Vert_{\mathrm{TV}} = 2 \sup_{A\in\mathfrak{B}(\mathcal{X})} \abs{\nu_1(A) - \nu_2(A)}.
\end{align}
\end{definition}
The total variation distance is easily verified to be a proper distance in that it satisfies non-negativity, discernability, symmetry, and the triangle inequality. The total variation distance can therefore be understood as the largest possible disagreement between the probabilities assigned to any measurable set by $\nu_1$ and $\nu_2$. The total variation norm has the following equivalent representations which are occasionally useful. 
\begin{proposition}
  Within the context of \cref{def:total-variation-norm}, the total variation distance between $\nu_1$ and $\nu_2$ is equivalently expressed as,
  \begin{align}
      \Vert\mu\Vert_\mathrm{TV} &= \sup_{f \in\mathcal{M}} \abs{\int_{\mathcal{X}} f(x) ~\nu_1(\mathrm{d}x) - \int_{\mathcal{X}} f(x) ~\nu_2(\mathrm{d}x)}
  \end{align}
  where $\mathcal{M} \defeq \set{f : \mathcal{X}\to\R ~\text{s.t.}~ \abs{f(x)} \leq 1~\forall~x\in\mathcal{X}}$.
\end{proposition}
For a proof of this result, and other equivalent characterizations of the total variation distance, we refer the interested reader to \cite{roberts-general-state-space,pollard_2001}.


==> Adaptation of the Independent Metropolis-Hastings Sampler with Normalizing Flow Proposals/appendices/violations-containment.tex <==
\clearpage
\section{Reasons for Violations of Containment}\label{app:violations-containment}

\subsubsection{Inexpressive Family} If the family of proposal densities is not sufficiently expressive, it may be that there does not exist any $M\geq 1$ satisfying $\log \pi(x) - \log\tilde{\pi}_{\theta}(x) < \log M$ for any $\theta$. For instance, on $\R^n$, if the proposal densities have tails that vanish exponentially quickly and the target density's tails diminish only polynomially, then the family of proposal densities is not sufficiently expressive for \cref{prop:containment-log-density} to hold; see \citet{pmlr-v119-jaini20a} for details on the tail behavior of normalizing flows. On the other hand, if the family of proposal distributions has a universality property (see, {\it inter alia} \citet{Kobyzev_2020}), then this concern can be alleviated.
\subsubsection{Mode Collapse} Proposal densities obtained through the minimization of certain loss functions, including $\mathbb{KL}(\tilde{\pi}_\theta\Vert\pi)$, may result in the modes of $\pi$ not being properly represented in the proposal density $\tilde{\pi}_\theta$. In the case of $\mathbb{KL}(\tilde{\pi}_\theta\Vert\pi)$, the mode-seeking behavior of the loss function can cause the mode-collapse phenomenon, which can invalidate the assumption of \cref{prop:containment-log-density}. One could alleviate this concern by targeting a tempered version of the target density or if one has confidence that mode collapse will not occur (for instance if the target density is unimodal).
\subsubsection{Unstable Loss} If the adaptations produced by attempting to minimize the loss function are ill-behaved (for instance if the step-size is too large, leading to divergent adaptations), then the sequence $(\Theta_n)_{n\in\mathbb{N}}$ may parameterize poor proposal densities which cause the failure of \cref{eq:containment-log-density}. If the algorithm relies of the convergence of the sequence $(\Theta_n)_{n\in\mathbb{N}}$, then ill-behaved adaptations may lead to a violation of ergodicity due to a failure of both containment and diminishing adaptation. 

==> Adaptation of the Independent Metropolis-Hastings Sampler with Normalizing Flow Proposals/figures/adaptive-mcmc.tex <==
\begin{figure}[t!]
\centering
\begin{tikzpicture}[
    node distance=2,thick,
    flow/.style={shorten >=3, shorten <=3, ->},
    znode/.style={circle,fill=black!10,minimum size=22,inner sep=0},
  ]

  \node[znode] (t0) {$\Theta_0$};

  \node[znode,below=0.4 of t0] (z0) {$X_0$};
  \node[znode,right=of z0] (z1) {$X_1$};
  \node[znode,above=0.4 of z1] (t1) {$\Theta_1$};

  \draw[flow] (z0) -- node[above,midway] {MH} (z1);

  \node[znode,right=of z1] (zi) {$X_n$};
  \node[znode,above=0.4 of zi] (tn) {$\Theta_n$};
  
  \draw[flow] (t0) --node[above,midway] {Adapt} (t1);
  \draw[flow] (t1) --node[above,midway] {Adapt} (tn);
  \draw[flow] (t1) --node[rectangle,fill=white,anchor=center,midway] {$\dots$} (tn);
  
  \draw[flow] (z1) -- node[above,midway] {MH} (zi);
  \draw[flow] (z1) --node[rectangle,fill=white,anchor=center,midway] {$\dots$} (zi);

  \node[outer sep=0,inner sep=0,below=0.2 of z0,label={below:$\tilde{\Pi}_{\Theta_0}$}] (f0) {\includegraphics[scale=0.1]{images/adaptive-mcmc-first.png}};
  % \node[outer sep=0,inner sep=0,left=1.0 of f0,label={below:Target}] (fk) {\includegraphics[scale=0.1]{images/adaptive-mcmc-target.png}};
  \node[outer sep=0,inner sep=0,below=0.2 of z1,label={below:$\tilde{\Pi}_{\Theta_1}$}] (fi) {\includegraphics[scale=0.1]{images/adaptive-mcmc-second.png}};
  \node[outer sep=0,inner sep=0,below=0.2 of zi,label={below:$\tilde{\Pi}_{\Theta_n}$}] (fk) {\includegraphics[scale=0.1]{images/adaptive-mcmc-target.png}};
  % \node[outer sep=0,inner sep=0,right=1.0 of fk,label={below:Samples}] (s) {\includegraphics[scale=0.1]{images/adaptive-mcmc-samples.png}};
  % \draw[flow] (fk) -- node[above,midway] {?} (s);
\end{tikzpicture}
\caption{This work examines the convergence of adaptive Markov chain Monte Carlo algorithms using the independent Metropolis-Hastings algorithm when the proposal distribution is parameterized by a normalizing flow. In this illustration, we seek to draw samples from a target distribution. We begin with an initial parameter $\Theta_0$ which parameterizes a simple proposal distribution, denoted $\tilde{\Pi}_{\Theta_0}$, which is a normalizing flow, and an initial state of the chain $X_0$; a sample from this proposal is accepted or rejected according to the Metropolis-Hastings criterion, yielding a transition to the state $X_1$. The parameters of the normalizing flow are thereafter adapted to produce a new proposal distribution $\tilde{\Pi}_{\Theta_1}$, which we hope is closer to the target distribution. Iterating this procedure we obtain both a sequence of states $(X_n)_{n\in\mathbb{N}}$ and a sequence of normalizing flow parameters $(\Theta_n)_{n\in\mathbb{N}}$. The principle question of this work is to establish when the sequence of states converges to the target density. \label{fig:adaptive-mcmc}}
\end{figure}

==> Adaptation of the Independent Metropolis-Hastings Sampler with Normalizing Flow Proposals/figures/brownian-bridge.tex <==
\begin{figure*}[t!]
    \centering
    \begin{subfigure}[t]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/brownian-bridge-ks.png}
        \caption{Kolmogorov-Smirnov Statistics}
        \label{subfig:brownian-bridge-ks}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/brownian-bridge-ess-per-second.png}
        \caption{ESS per Second}
        \label{subfig:brownian-bridge-ess}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/brownian-bridge-ap.png}
        \caption{Acceptance Probability}
        \label{subfig:brownian-bridge-ap}
    \end{subfigure}
    \caption{Result of the Brownian bridge experiment. In assessing ergodicity according to the distribution of Kolmogorov-Smirnov statistics along random one-dimensional sub-spaces, the methods based on the independent Metropolis-Hastings algorithm and preconditioned Langevin dynamcis perform best. Langevin dynamics struggles in this posterior due to the multi-scale phenomena present in this distribution. In terms of the effective sample size per second of computation, the near-independent proposals and high acceptance rate of the independent Metropolis-Hastings sampler cause these algorithms to dominate. We also show the acceptance probability of the adaptive methods; we observe that the independent Metropolis-Hastings procedures enjoy adaptations that cause the acceptance probability to consistently improve over the course of learning.}
    \label{fig:brownian-bridge}
\end{figure*}

==> Adaptation of the Independent Metropolis-Hastings Sampler with Normalizing Flow Proposals/figures/field-model-samples.tex <==
\begin{figure*}[t!]
    \centering
    \begin{subfigure}[t]{\textwidth}
        \centering
        \includegraphics[width=\textwidth,trim={2.5cm 0 2.5cm 0},clip]{images/Samples_MALA_13-10-2021_stochmetromalangevin_phi4_N100_a0_10_b0_00e+00_beta20_00_priorcoupled_rposinit0_2_5blocks1deep_1149510_2.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{01\textwidth}
        \centering
        \includegraphics[width=\textwidth,trim={2.5cm 0 2.5cm 0},clip]{images/Samples_Adapt_13-10-2021_stochmetromalangevin_phi4_N100_a0_10_b0_00e+00_beta20_00_priorcoupled_rposinit0_2_5blocks1deep_1149510_2.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{\textwidth}
        \centering
        \includegraphics[width=\textwidth,trim={2.5cm 0 2.5cm 0},clip]{images/Samples_NF_13-10-2021_stochmetromalangevin_phi4_N100_a0_10_b0_00e+00_beta20_00_priorcoupled_rposinit0_2_5blocks1deep_1149510_2.png}
    \end{subfigure}
    \caption{Samples and proposals in the $\phi^4$ field experiment.}
    \label{fig:field-model-samples}
\end{figure*}


==> Adaptation of the Independent Metropolis-Hastings Sampler with Normalizing Flow Proposals/figures/field-model.tex <==

\begin{figure*}[t!]
    \centering
    \begin{subfigure}[t]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/KS_10chains_fullchains_13-10-2021_stochmetromalangevin_phi4_N100_a0_10_b0_00e+00_beta20_00_priorcoupled_rposinit0_2_5blocks1deep_1149510_2.png}
        \caption{Kolmogorov-Smirnov Statistics}
        \label{subfigfield-model-ks}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/ESS_13-10-2021_stochmetromalangevin_phi4_1149510_2_length1000_burn40000_early_late.png}
        \caption{ESS per Second}
        \label{subfig:field-model-ess}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/Accs_13-10-2021_stochmetromalangevin_phi4_N100_a0_10_b0_00e+00_beta20_00_priorcoupled_rposinit0_2_5blocks1deep_1149510_2.png}
        \caption{Acceptance Probability}
        \label{subfig:field-model-ap}
    \end{subfigure}
    \caption{Results of the $\phi^4$ field experiment.
    As Langevin dynamics is unable to mix between the two modes, the better ergodicity of the independent Metropolis Hastings algorithm is reflected in Kolmogorov-Smirnov statistics as expected. The single chain Langevin has  poorer ergodicity than its parallel chain equivalent, while for the I.M.H. a single chain approaches the ergodicity of the parallel setting. The Effective Sample Sizes are reported for chains of $1000$ steps extracted at burn-in, after $4\times 10 ^4$ iterations (early) and (late) when the NF proposal acceptance probability has reached ~50\%. Note that periodic jumps in acceptance correspond to iterations where learning rate was decreased. 
    }
    \label{fig:field-model}
\end{figure*}


==> Adaptation of the Independent Metropolis-Hastings Sampler with Normalizing Flow Proposals/figures/simultaneous-uniform-ergodicity-containment.tex <==
\begin{figure*}[t!]
    \centering
    \begin{subfigure}[t]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/simultaneous-uniform-ergodicity-failure.png}
        \caption{Failure of simultaneous uniform ergodicity}
        \label{subfig:simultaneous-uniform-ergodicity-failure}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/simultaneous-uniform-ergodicity-mixing.png}
        \caption{Simultaneous uniform ergodicity via mixing}
        \label{subfig:simultaneous-uniform-ergodicity-mixing}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/containment-bound.png}
        \caption{Containment}
        \label{subfig:containment-bound}
    \end{subfigure}
    \caption{Establishing ergodicity of an adaptive chain sampler with non-independent adaptations requires showing that either the simultaneous uniform ergodicity or containment properties hold. In \cref{subfig:simultaneous-uniform-ergodicity-failure}, we show how adaptations can produce a catastrophic failure of ergodicity by visualizing the log-densities of the target distribution and the adaptive proposal distributions: the proposal distribution becomes increasingly concentrated, meaning that there is no uniform bound on the $\epsilon$-mixing time. On a compact space, this phenomenon can be defeated by mixing the normalizing flow with a fixed distribution with full support; we visualize this effect in \cref{subfig:simultaneous-uniform-ergodicity-mixing}. An alternative to mixing is to look toward the containment property. When there is a finite upper bound on the difference between the target density and the proposal density, containment is implied for the independent Metropolis-Hastings sampler. In \cref{subfig:containment-bound}, containment is visualized as the fact that all of the log-densities of the proposal distributions are uniformly greater than the target log-density translated down by some quantity greater than zero (dotted blue line).}
\end{figure*}

==> Adaptation of the Independent Metropolis-Hastings Sampler with Normalizing Flow Proposals/figures/two-dimensional.tex <==
\begin{figure*}[t!]
    \centering
    \begin{subfigure}[t]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/multimodal-ap.png}
        \caption{(Multimodal) Acc. Prob.}
        \label{subfig:simple-multimodal-ap}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/multimodal-ks.png}
        \caption{(Multimodal) KS}
        \label{subfig:simple-multimodal-ks}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/neal-funnel-ks.png}
        \caption{(Neal Funnel) KS}
        \label{subfig:simple-neal-funnel-ks}
    \end{subfigure}
    \caption{Examination of the performance of MCMC methods on sampling from the multimodal and Neal funnel distributions. Both adaptive methods enjoy increasing acceptance rates in the multimodal distribution as a function of sampling iteration, but only the adaptive independent Metropolis-Hastings algorithm exhibits ergodicity for this distribution. Indeed, for the adaptive random walk and Langevin sampling methods, which are based on local updates, the multimodal distribution poses distinct challenges. In fact, both methods get stuck in one of the modes. By contrast, the adaptive independent Metropolis-Hastings samplers exhibit the best ergodicity of all methods considered. In Neal's funnel distribution, the adaptive independent Metropolis-Hastings algorithm possesses the best ergodicity.}
    \label{fig:simple-two-dimensional}
\end{figure*}

==> Adaptation of the Independent Metropolis-Hastings Sampler with Normalizing Flow Proposals/figures/violations-of-stationarity.tex <==
\begin{figure*}[t!]
    \centering
    \begin{subfigure}[t]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/adaptive-stationarity-violate-True-num-steps-100.png}
        \caption{100 Steps}
        \label{subfig:stationarity-violation-100}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/adaptive-stationarity-violate-True-num-steps-10000.png}
        \caption{10,000 Steps}
        \label{subfig:stationarity-violation-10000}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/adaptive-stationarity-kl.png}
        \caption{Forward KL divergence by Step}
        \label{subfig:stationarity-violation-kl}
    \end{subfigure}
    \caption{Examinations of the violations of stationarity that result by maximizing the pseudo-likelihood of the accepted samples as an adaptation mechanism. After one-hundred steps of adaptation, one clearly perceives that the distribution of states does {\it not} follow the target distribution. However, after ten-thousand steps, the distribution of state is closer to the target distribution. We also show the KL divergence between the target distribution at the proposal distribution according to the number of steps of the chain. Results are computed over one-million random simulations.}
    \label{fig:stationarity-violation}
\end{figure*}
